Signatures of Non-thermal Dark Matter with Kination and Early Matter Domination: Gravitational Waves versus Laboratory Searches

The non-thermal production of dark matter (DM) usually requires very tiny couplings of the dark sector with the visible sector and therefore is notoriously challenging to hunt in laboratory experiments. Here we propose a novel pathway to test such a production in the context of a non-standard cosmological history, using both gravitational wave (GW) and laboratory searches. We investigate the formation of DM from the decay of a scalar field that we dub as the reheaton, as it also reheats the Universe when it decays. We consider the possibility that the Universe undergoes a phase %of kination with \textit{kination-like} stiff equation-of-state ($w_{\rm kin}>1/3$) before the reheaton dominates the energy density of the Universe and eventually decays into Standard Model and DM particles. We then study how first-order tensor perturbations generated during inflation, the amplitude of which may get amplified during the kination era and lead to detectable GW signals. Demanding that the reheaton produces the observed DM relic density, we show that the reheaton's lifetime and branching fractions are dictated by the cosmological scenario. In particular, we show that it is long-lived and can be searched by various experiments such as DUNE, FASER, FASER-II, MATHUSLA, SHiP, etc. We also identify the parameter space which leads to complementary observables for GW detectors such as LISA and u-DECIGO. In particular we find that a kination-like period with an equation-of-state parameter $w_{\rm kin}\approx 0.5$ and a reheaton mass $\mathcal O(0.5-5)$ GeV and a DM mass of $\mathcal O (10-100)$ keV may lead to sizeable imprints in both kinds of searches.

==> backup/main_old <==
@article{Buchmuller:2014pla,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Wieck, Clemens",
    title = "{Large-Field Inflation and Supersymmetry Breaking}",
    eprint = "1407.0253",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-14-100, CPHT-RR037.0614",
    doi = "10.1007/JHEP09(2014)053",
    journal = "JHEP",
    volume = "09",
    pages = "053",
    year = "2014"
}

@article{Buchmuller:2015oma,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Westphal, Alexander and Wieck, Clemens and Winkler, Martin Wolfgang",
    title = "{Challenges for Large-Field Inflation and Moduli Stabilization}",
    eprint = "1501.05812",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-15-014, CPHT-RR002.0115",
    doi = "10.1007/JHEP04(2015)058",
    journal = "JHEP",
    volume = "04",
    pages = "058",
    year = "2015"
}

@article{Argurio:2017joe,
    author = "Argurio, Riccardo and Coone, Dries and Heurtier, Lucien and Mariotti, Alberto",
    title = "{Sgoldstino-less inflation and low energy SUSY breaking}",
    eprint = "1705.06788",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2017/07/047",
    journal = "JCAP",
    volume = "07",
    pages = "047",
    year = "2017"
}

@article{Heurtier:2019eou,
    author = "Heurtier, Lucien and Huang, Fei",
    title = "{Inflaton portal to a highly decoupled EeV dark matter particle}",
    eprint = "1905.05191",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.100.043507",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "4",
    pages = "043507",
    year = "2019"
}

@article{Enqvist:2016mqj,
    author = "Enqvist, Kari and Karciauskas, Mindaugas and Lebedev, Oleg and Rusak, Stanislav and Zatta, Marco",
    title = "{Postinflationary vacuum instability and Higgs-inflaton couplings}",
    eprint = "1608.08848",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2016/11/025",
    journal = "JCAP",
    volume = "11",
    pages = "025",
    year = "2016"
}

@article{Akrami:2017cir,
    author = "Akrami, Yashar and Kallosh, Renata and Linde, Andrei and Vardanyan, Valeri",
    title = "{Dark energy, $\alpha$-attractors, and large-scale structure surveys}",
    eprint = "1712.09693",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2018/06/041",
    journal = "JCAP",
    volume = "06",
    pages = "041",
    year = "2018"
}

@article{Dimopoulos:2001ix,
    author = "Dimopoulos, Konstantinos and Valle, J. W. F.",
    title = "{Modeling quintessential inflation}",
    eprint = "astro-ph/0111417",
    archivePrefix = "arXiv",
    reportNumber = "IFIC-01-49, LANCS-01-21-11",
    doi = "10.1016/S0927-6505(02)00115-9",
    journal = "Astropart. Phys.",
    volume = "18",
    pages = "287--306",
    year = "2002"
}

@article{Ellis:2020krl,
    author = "Ellis, John and Nanopoulos, Dimitri V. and Olive, Keith A. and Verner, Sarunas",
    title = "{Non-Oscillatory No-Scale Inflation}",
    eprint = "2008.09099",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMN-TH-3924/20, FTPI-MINN-20/27, KCL-PH-TH/2020-38,
  CERN-TH-2020-123, ACT-05-20, MI-TH-2020",
    doi = "10.1088/1475-7516/2021/03/052",
    journal = "JCAP",
    volume = "03",
    pages = "052",
    year = "2021"
}

@article{Gouttenoire:2021jhk,
    author = "Gouttenoire, Yann and Servant, Geraldine and Simakachorn, Peera",
    title = "{Kination cosmology from scalar fields and gravitational-wave signatures}",
    eprint = "2111.01150",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 21-134",
    month = "11",
    year = "2021"
}

@article{Planck:2018vyg,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}

@article{Barman:2022njh,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Probing pre-BBN era with Scale Invarint FIMP}",
    eprint = "2203.13269",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-712FT",
    month = "3",
    year = "2022"
}

@article{Barman:2021lot,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Scale invariant FIMP miracle}",
    eprint = "2109.03259",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-698FT",
    doi = "10.1088/1475-7516/2022/03/003",
    journal = "JCAP",
    volume = "03",
    number = "03",
    pages = "003",
    year = "2022"
}

@article{Feng:2017vli,
    author = "Feng, Jonathan L. and Galon, Iftah and Kling, Felix and Trojanowski, Sebastian",
    title = "{Dark Higgs bosons at the ForwArd Search ExpeRiment}",
    eprint = "1710.09387",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2017-12",
    doi = "10.1103/PhysRevD.97.055034",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "5",
    pages = "055034",
    year = "2018"
}

@article{FASER:2018eoc,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER\textquoteright{}s physics reach for long-lived particles}",
    eprint = "1811.12522",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2018-19, KYUSHU-RCAPP-2018-06",
    doi = "10.1103/PhysRevD.99.095011",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "9",
    pages = "095011",
    year = "2019"
}

@article{FASER:2018bac,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{Technical Proposal for FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1812.09139",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-LHCC-2018-036, LHCC-P-013, UCI-TR-2018-22, KYUSHU-RCAPP-2018-07",
    month = "12",
    year = "2018"
}

@article{FASER:2019aik,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1901.04468",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2019-01, KYUSHU-RCAPP-2018-08",
    month = "1",
    year = "2019"
}

@article{DUNE:2015lol,
    author = "Acciarri, R. and others",
    collaboration = "DUNE",
    title = "{Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE)}: {Conceptual Design Report, Volume 2: The Physics Program for DUNE at LBNF}",
    eprint = "1512.06148",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-DESIGN-2016-02",
    month = "12",
    year = "2015"
}

@article{Berryman:2019dme,
    author = "Berryman, Jeffrey M. and de Gouvea, Andre and Fox, Patrick J and Kayser, Boris Jules and Kelly, Kevin James and Raaf, Jennifer Lynne",
    title = "{Searches for Decays of New Particles in the DUNE Multi-Purpose Near Detector}",
    eprint = "1912.07622",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-19-607-ND-T, NUHEP-TH/19-16",
    doi = "10.1007/JHEP02(2020)174",
    journal = "JHEP",
    volume = "02",
    pages = "174",
    year = "2020"
}

@article{Batell:2020vqn,
    author = "Batell, Brian and Evans, Jared A. and Gori, Stefania and Rai, Mudit",
    title = "{Dark Scalars and Heavy Neutral Leptons at DarkQuest}",
    eprint = "2008.08108",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2021)049",
    journal = "JHEP",
    volume = "05",
    pages = "049",
    year = "2021"
}

@article{Bernardi:1985ny,
    author = "Bernardi, G. and others",
    title = "{Search for Neutrino Decay}",
    reportNumber = "CERN-EP/85-177",
    doi = "10.1016/0370-2693(86)91602-3",
    journal = "Phys. Lett. B",
    volume = "166",
    pages = "479--483",
    year = "1986"
}

@article{Gorbunov:2021ccu,
    author = "Gorbunov, Dmitry and Krasnov, Igor and Suvorov, Sergey",
    title = "{Constraints on light scalars from PS191 results}",
    eprint = "2105.11102",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "INR-TH-2021-012",
    doi = "10.1016/j.physletb.2021.136524",
    journal = "Phys. Lett. B",
    volume = "820",
    pages = "136524",
    year = "2021"
}

@article{Curtin:2018mvb,
    author = "Curtin, David and others",
    title = "{Long-Lived Particles at the Energy Frontier: The MATHUSLA Physics Case}",
    eprint = "1806.07396",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-264-T",
    doi = "10.1088/1361-6633/ab28d6",
    journal = "Rept. Prog. Phys.",
    volume = "82",
    number = "11",
    pages = "116201",
    year = "2019"
}

@article{SHiP:2015vad,
    author = "Anelli, M. and others",
    collaboration = "SHiP",
    title = "{A facility to Search for Hidden Particles (SHiP) at the CERN SPS}",
    eprint = "1504.04956",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-SPSC-2015-016, SPSC-P-350",
    month = "4",
    year = "2015"
}

==> backup/main_old_v2 <==
@article{Buchmuller:2014pla,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Wieck, Clemens",
    title = "{Large-Field Inflation and Supersymmetry Breaking}",
    eprint = "1407.0253",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-14-100, CPHT-RR037.0614",
    doi = "10.1007/JHEP09(2014)053",
    journal = "JHEP",
    volume = "09",
    pages = "053",
    year = "2014"
}


@article{Buchmuller:2015oma,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Westphal, Alexander and Wieck, Clemens and Winkler, Martin Wolfgang",
    title = "{Challenges for Large-Field Inflation and Moduli Stabilization}",
    eprint = "1501.05812",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-15-014, CPHT-RR002.0115",
    doi = "10.1007/JHEP04(2015)058",
    journal = "JHEP",
    volume = "04",
    pages = "058",
    year = "2015"
}


@article{Argurio:2017joe,
    author = "Argurio, Riccardo and Coone, Dries and Heurtier, Lucien and Mariotti, Alberto",
    title = "{Sgoldstino-less inflation and low energy SUSY breaking}",
    eprint = "1705.06788",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2017/07/047",
    journal = "JCAP",
    volume = "07",
    pages = "047",
    year = "2017"
}


@article{Heurtier:2019eou,
    author = "Heurtier, Lucien and Huang, Fei",
    title = "{Inflaton portal to a highly decoupled EeV dark matter particle}",
    eprint = "1905.05191",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.100.043507",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "4",
    pages = "043507",
    year = "2019"
}


@article{Enqvist:2016mqj,
    author = "Enqvist, Kari and Karciauskas, Mindaugas and Lebedev, Oleg and Rusak, Stanislav and Zatta, Marco",
    title = "{Postinflationary vacuum instability and Higgs-inflaton couplings}",
    eprint = "1608.08848",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2016/11/025",
    journal = "JCAP",
    volume = "11",
    pages = "025",
    year = "2016"
}


@article{Akrami:2017cir,
    author = "Akrami, Yashar and Kallosh, Renata and Linde, Andrei and Vardanyan, Valeri",
    title = "{Dark energy, $\alpha$-attractors, and large-scale structure surveys}",
    eprint = "1712.09693",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2018/06/041",
    journal = "JCAP",
    volume = "06",
    pages = "041",
    year = "2018"
}


@article{Dimopoulos:2001ix,
    author = "Dimopoulos, Konstantinos and Valle, J. W. F.",
    title = "{Modeling quintessential inflation}",
    eprint = "astro-ph/0111417",
    archivePrefix = "arXiv",
    reportNumber = "IFIC-01-49, LANCS-01-21-11",
    doi = "10.1016/S0927-6505(02)00115-9",
    journal = "Astropart. Phys.",
    volume = "18",
    pages = "287--306",
    year = "2002"
}


@article{Ellis:2020krl,
    author = "Ellis, John and Nanopoulos, Dimitri V. and Olive, Keith A. and Verner, Sarunas",
    title = "{Non-Oscillatory No-Scale Inflation}",
    eprint = "2008.09099",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMN-TH-3924/20, FTPI-MINN-20/27, KCL-PH-TH/2020-38,
  CERN-TH-2020-123, ACT-05-20, MI-TH-2020",
    doi = "10.1088/1475-7516/2021/03/052",
    journal = "JCAP",
    volume = "03",
    pages = "052",
    year = "2021"
}


@article{Gouttenoire:2021jhk,
    author = "Gouttenoire, Yann and Servant, Geraldine and Simakachorn, Peera",
    title = "{Kination cosmology from scalar fields and gravitational-wave signatures}",
    eprint = "2111.01150",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 21-134",
    month = "11",
    year = "2021"
}


@article{Planck:2018vyg,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Watanabe:2006qe,
    author = "Watanabe, Yuki and Komatsu, Eiichiro",
    title = "{Improved Calculation of the Primordial Gravitational Wave Spectrum in the Standard Model}",
    eprint = "astro-ph/0604176",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.73.123515",
    journal = "Phys. Rev. D",
    volume = "73",
    pages = "123515",
    year = "2006"
}


@article{Saikawa:2018rcs,
    author = "Saikawa, Ken'ichi and Shirai, Satoshi",
    title = "{Primordial gravitational waves, precisely: The role of thermodynamics in the Standard Model}",
    eprint = "1803.01038",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPMU18-0037, MPP-2018-19",
    doi = "10.1088/1475-7516/2018/05/035",
    journal = "JCAP",
    volume = "05",
    pages = "035",
    year = "2018"
}


@article{Bernal:2019lpc,
    author = "Bernal, Nicol\'as and Hajkarim, Fazlollah",
    title = "{Primordial Gravitational Waves in Nonstandard Cosmologies}",
    eprint = "1905.10410",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.100.063502",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "6",
    pages = "063502",
    year = "2019"
}


@article{Weinberg:2003ur,
    author = "Weinberg, Steven",
    title = "{Damping of tensor modes in cosmology}",
    eprint = "astro-ph/0306304",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-02-03",
    doi = "10.1103/PhysRevD.69.023503",
    journal = "Phys. Rev. D",
    volume = "69",
    pages = "023503",
    year = "2004"
}


@article{Drees:2015exa,
    author = "Drees, Manuel and Hajkarim, Fazlollah and Schmitz, Ernany Rossi",
    title = "{The Effects of QCD Equation of State on the Relic Density of WIMP Dark Matter}",
    eprint = "1503.03513",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2015/06/025",
    journal = "JCAP",
    volume = "06",
    pages = "025",
    year = "2015"
}


@article{Aghanim:2018eyx,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Thrane:2013oya,
    author = "Thrane, Eric and Romano, Joseph D.",
    title = "{Sensitivity curves for searches for gravitational-wave backgrounds}",
    eprint = "1310.5300",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1103/PhysRevD.88.124032",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "12",
    pages = "124032",
    year = "2013"
}


@article{Caprini:2015zlo,
    author = "Caprini, Chiara and others",
    title = "{Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions}",
    eprint = "1512.06239",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-15-246",
    doi = "10.1088/1475-7516/2016/04/001",
    journal = "JCAP",
    volume = "04",
    pages = "001",
    year = "2016"
}


@article{Feng:2017vli,
    author = "Feng, Jonathan L. and Galon, Iftah and Kling, Felix and Trojanowski, Sebastian",
    title = "{Dark Higgs bosons at the ForwArd Search ExpeRiment}",
    eprint = "1710.09387",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2017-12",
    doi = "10.1103/PhysRevD.97.055034",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "5",
    pages = "055034",
    year = "2018"
}


@article{FASER:2018eoc,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER\textquoteright{}s physics reach for long-lived particles}",
    eprint = "1811.12522",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2018-19, KYUSHU-RCAPP-2018-06",
    doi = "10.1103/PhysRevD.99.095011",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "9",
    pages = "095011",
    year = "2019"
}


@article{FASER:2018bac,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{Technical Proposal for FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1812.09139",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-LHCC-2018-036, LHCC-P-013, UCI-TR-2018-22, KYUSHU-RCAPP-2018-07",
    month = "12",
    year = "2018"
}


@article{FASER:2019aik,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1901.04468",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2019-01, KYUSHU-RCAPP-2018-08",
    month = "1",
    year = "2019"
}


@article{DUNE:2015lol,
    author = "Acciarri, R. and others",
    collaboration = "DUNE",
    title = "{Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE)}: {Conceptual Design Report, Volume 2: The Physics Program for DUNE at LBNF}",
    eprint = "1512.06148",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-DESIGN-2016-02",
    month = "12",
    year = "2015"
}


@article{Berryman:2019dme,
    author = "Berryman, Jeffrey M. and de Gouvea, Andre and Fox, Patrick J and Kayser, Boris Jules and Kelly, Kevin James and Raaf, Jennifer Lynne",
    title = "{Searches for Decays of New Particles in the DUNE Multi-Purpose Near Detector}",
    eprint = "1912.07622",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-19-607-ND-T, NUHEP-TH/19-16",
    doi = "10.1007/JHEP02(2020)174",
    journal = "JHEP",
    volume = "02",
    pages = "174",
    year = "2020"
}


@article{Batell:2020vqn,
    author = "Batell, Brian and Evans, Jared A. and Gori, Stefania and Rai, Mudit",
    title = "{Dark Scalars and Heavy Neutral Leptons at DarkQuest}",
    eprint = "2008.08108",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2021)049",
    journal = "JHEP",
    volume = "05",
    pages = "049",
    year = "2021"
}


@article{Curtin:2018mvb,
    author = "Curtin, David and others",
    title = "{Long-Lived Particles at the Energy Frontier: The MATHUSLA Physics Case}",
    eprint = "1806.07396",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-264-T",
    doi = "10.1088/1361-6633/ab28d6",
    journal = "Rept. Prog. Phys.",
    volume = "82",
    number = "11",
    pages = "116201",
    year = "2019"
}


@article{Bernardi:1985ny,
    author = "Bernardi, G. and others",
    title = "{Search for Neutrino Decay}",
    reportNumber = "CERN-EP/85-177",
    doi = "10.1016/0370-2693(86)91602-3",
    journal = "Phys. Lett. B",
    volume = "166",
    pages = "479--483",
    year = "1986"
}


@article{Gorbunov:2021ccu,
    author = "Gorbunov, Dmitry and Krasnov, Igor and Suvorov, Sergey",
    title = "{Constraints on light scalars from PS191 results}",
    eprint = "2105.11102",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "INR-TH-2021-012",
    doi = "10.1016/j.physletb.2021.136524",
    journal = "Phys. Lett. B",
    volume = "820",
    pages = "136524",
    year = "2021"
}


@article{SHiP:2015vad,
    author = "Anelli, M. and others",
    collaboration = "SHiP",
    title = "{A facility to Search for Hidden Particles (SHiP) at the CERN SPS}",
    eprint = "1504.04956",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-SPSC-2015-016, SPSC-P-350",
    month = "4",
    year = "2015"
}


@article{Barman:2022njh,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Probing pre-BBN era with Scale Invarint FIMP}",
    eprint = "2203.13269",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-712FT",
    month = "3",
    year = "2022"
}


@article{Barman:2021lot,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Scale invariant FIMP miracle}",
    eprint = "2109.03259",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-698FT",
    doi = "10.1088/1475-7516/2022/03/003",
    journal = "JCAP",
    volume = "03",
    number = "03",
    pages = "003",
    year = "2022"
}


==> backup/main_old_v3 <==
@article{Buchmuller:2014pla,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Wieck, Clemens",
    title = "{Large-Field Inflation and Supersymmetry Breaking}",
    eprint = "1407.0253",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-14-100, CPHT-RR037.0614",
    doi = "10.1007/JHEP09(2014)053",
    journal = "JHEP",
    volume = "09",
    pages = "053",
    year = "2014"
}


@article{Buchmuller:2015oma,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Westphal, Alexander and Wieck, Clemens and Winkler, Martin Wolfgang",
    title = "{Challenges for Large-Field Inflation and Moduli Stabilization}",
    eprint = "1501.05812",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-15-014, CPHT-RR002.0115",
    doi = "10.1007/JHEP04(2015)058",
    journal = "JHEP",
    volume = "04",
    pages = "058",
    year = "2015"
}


@article{Argurio:2017joe,
    author = "Argurio, Riccardo and Coone, Dries and Heurtier, Lucien and Mariotti, Alberto",
    title = "{Sgoldstino-less inflation and low energy SUSY breaking}",
    eprint = "1705.06788",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2017/07/047",
    journal = "JCAP",
    volume = "07",
    pages = "047",
    year = "2017"
}


@article{Heurtier:2019eou,
    author = "Heurtier, Lucien and Huang, Fei",
    title = "{Inflaton portal to a highly decoupled EeV dark matter particle}",
    eprint = "1905.05191",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.100.043507",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "4",
    pages = "043507",
    year = "2019"
}


@article{Enqvist:2016mqj,
    author = "Enqvist, Kari and Karciauskas, Mindaugas and Lebedev, Oleg and Rusak, Stanislav and Zatta, Marco",
    title = "{Postinflationary vacuum instability and Higgs-inflaton couplings}",
    eprint = "1608.08848",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2016/11/025",
    journal = "JCAP",
    volume = "11",
    pages = "025",
    year = "2016"
}


@article{Akrami:2017cir,
    author = "Akrami, Yashar and Kallosh, Renata and Linde, Andrei and Vardanyan, Valeri",
    title = "{Dark energy, $\alpha$-attractors, and large-scale structure surveys}",
    eprint = "1712.09693",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2018/06/041",
    journal = "JCAP",
    volume = "06",
    pages = "041",
    year = "2018"
}


@article{Dimopoulos:2001ix,
    author = "Dimopoulos, Konstantinos and Valle, J. W. F.",
    title = "{Modeling quintessential inflation}",
    eprint = "astro-ph/0111417",
    archivePrefix = "arXiv",
    reportNumber = "IFIC-01-49, LANCS-01-21-11",
    doi = "10.1016/S0927-6505(02)00115-9",
    journal = "Astropart. Phys.",
    volume = "18",
    pages = "287--306",
    year = "2002"
}


@article{Ellis:2020krl,
    author = "Ellis, John and Nanopoulos, Dimitri V. and Olive, Keith A. and Verner, Sarunas",
    title = "{Non-Oscillatory No-Scale Inflation}",
    eprint = "2008.09099",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMN-TH-3924/20, FTPI-MINN-20/27, KCL-PH-TH/2020-38,
  CERN-TH-2020-123, ACT-05-20, MI-TH-2020",
    doi = "10.1088/1475-7516/2021/03/052",
    journal = "JCAP",
    volume = "03",
    pages = "052",
    year = "2021"
}


@article{Gouttenoire:2021jhk,
    author = "Gouttenoire, Yann and Servant, Geraldine and Simakachorn, Peera",
    title = "{Kination cosmology from scalar fields and gravitational-wave signatures}",
    eprint = "2111.01150",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 21-134",
    month = "11",
    year = "2021"
}


@article{Planck:2018vyg,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Watanabe:2006qe,
    author = "Watanabe, Yuki and Komatsu, Eiichiro",
    title = "{Improved Calculation of the Primordial Gravitational Wave Spectrum in the Standard Model}",
    eprint = "astro-ph/0604176",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.73.123515",
    journal = "Phys. Rev. D",
    volume = "73",
    pages = "123515",
    year = "2006"
}


@article{Saikawa:2018rcs,
    author = "Saikawa, Ken'ichi and Shirai, Satoshi",
    title = "{Primordial gravitational waves, precisely: The role of thermodynamics in the Standard Model}",
    eprint = "1803.01038",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPMU18-0037, MPP-2018-19",
    doi = "10.1088/1475-7516/2018/05/035",
    journal = "JCAP",
    volume = "05",
    pages = "035",
    year = "2018"
}


@article{Bernal:2019lpc,
    author = "Bernal, Nicol\'as and Hajkarim, Fazlollah",
    title = "{Primordial Gravitational Waves in Nonstandard Cosmologies}",
    eprint = "1905.10410",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.100.063502",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "6",
    pages = "063502",
    year = "2019"
}


@article{Weinberg:2003ur,
    author = "Weinberg, Steven",
    title = "{Damping of tensor modes in cosmology}",
    eprint = "astro-ph/0306304",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-02-03",
    doi = "10.1103/PhysRevD.69.023503",
    journal = "Phys. Rev. D",
    volume = "69",
    pages = "023503",
    year = "2004"
}


@article{Drees:2015exa,
    author = "Drees, Manuel and Hajkarim, Fazlollah and Schmitz, Ernany Rossi",
    title = "{The Effects of QCD Equation of State on the Relic Density of WIMP Dark Matter}",
    eprint = "1503.03513",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2015/06/025",
    journal = "JCAP",
    volume = "06",
    pages = "025",
    year = "2015"
}


@article{Aghanim:2018eyx,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Starobinsky:1985ww,
    author = "Starobinsky, A. A.",
    title = "{Cosmic Background Anisotropy Induced by Isotropic Flat-Spectrum Gravitational-Wave Perturbations}",
    journal = "Sov. Astron. Lett.",
    volume = "11",
    pages = "133",
    year = "1985"
}


@article{Schmitz:2020syl,
    author = "Schmitz, Kai",
    title = "{New Sensitivity Curves for Gravitational-Wave Signals from Cosmological Phase Transitions}",
    eprint = "2002.04615",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-018",
    doi = "10.1007/JHEP01(2021)097",
    journal = "JHEP",
    volume = "01",
    pages = "097",
    year = "2021"
}


@article{McLaughlin:2013ira,
    author = "McLaughlin, Maura A.",
    title = "{The North American Nanohertz Observatory for Gravitational Waves}",
    eprint = "1310.0758",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/0264-9381/30/22/224008",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224008",
    year = "2013"
}


@article{NANOGRAV:2018hou,
    author = "Arzoumanian, Z. and others",
    collaboration = "NANOGRAV",
    title = "{The NANOGrav 11-year Data Set: Pulsar-timing Constraints On The Stochastic Gravitational-wave Background}",
    eprint = "1801.02617",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.HE",
    doi = "10.3847/1538-4357/aabd3b",
    journal = "Astrophys. J.",
    volume = "859",
    number = "1",
    pages = "47",
    year = "2018"
}


@article{Aggarwal:2018mgp,
    author = "Aggarwal, K. and others",
    title = "{The NANOGrav 11-Year Data Set: Limits on Gravitational Waves from Individual Supermassive Black Hole Binaries}",
    eprint = "1812.11585",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.GA",
    doi = "10.3847/1538-4357/ab2236",
    journal = "Astrophys. J.",
    volume = "880",
    pages = "2",
    year = "2019"
}


@article{Brazier:2019mmu,
    author = "Brazier, A. and others",
    title = "{The NANOGrav Program for Gravitational Waves and Fundamental Physics}",
    eprint = "1908.05356",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "8",
    year = "2019"
}


@article{Manchester:2012za,
    author = "Manchester, R. N. and others",
    title = "{The Parkes Pulsar Timing Array Project}",
    eprint = "1210.6130",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1017/pasa.2012.017",
    journal = "Publ. Astron. Soc. Austral.",
    volume = "30",
    pages = "17",
    year = "2013"
}


@article{Shannon:2015ect,
    author = "Shannon, R. M. and others",
    title = "{Gravitational waves from binary supermassive black holes missing in pulsar observations}",
    eprint = "1509.07320",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1126/science.aab1910",
    journal = "Science",
    volume = "349",
    number = "6255",
    pages = "1522--1525",
    year = "2015"
}


@article{Kramer:2013kea,
    author = "Kramer, Michael and Champion, David J.",
    title = "{The European Pulsar Timing Array and the Large European Array for Pulsars}",
    doi = "10.1088/0264-9381/30/22/224009",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224009",
    year = "2013"
}


@article{Lentati:2015qwp,
    author = "Lentati, L. and others",
    title = "{European Pulsar Timing Array Limits On An Isotropic Stochastic Gravitational-Wave Background}",
    eprint = "1504.03692",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stv1538",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "453",
    number = "3",
    pages = "2576--2598",
    year = "2015"
}


@article{Babak:2015lua,
    author = "Babak, Stanislav and others",
    title = "{European Pulsar Timing Array Limits on Continuous Gravitational Waves from Individual Supermassive Black Hole Binaries}",
    eprint = "1509.02165",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stv2092",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "455",
    number = "2",
    pages = "1665--1679",
    year = "2016"
}


@article{Hobbs:2009yy,
    author = "Hobbs, G. and others",
    editor = "Marka, Zsuzsa and Marka, Szabolcs",
    title = "{The international pulsar timing array project: using pulsars as a gravitational wave detector}",
    eprint = "0911.5206",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.SR",
    doi = "10.1088/0264-9381/27/8/084013",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "084013",
    year = "2010"
}


@article{Manchester:2013ndt,
    author = "Manchester, R. N.",
    title = "{The International Pulsar Timing Array}",
    eprint = "1309.7392",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/0264-9381/30/22/224010",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224010",
    year = "2013"
}


@article{Verbiest:2016vem,
    author = "Verbiest, J. P. W. and others",
    title = "{The International Pulsar Timing Array: First Data Release}",
    eprint = "1602.03640",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1093/mnras/stw347",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "458",
    number = "2",
    pages = "1267--1288",
    year = "2016"
}


@article{Hazboun:2018wpv,
    author = "Hazboun, Jeffrey S. and Mingarelli, Chiara M. F. and Lee, Kejia",
    title = "{The Second International Pulsar Timing Array Mock Data Challenge}",
    eprint = "1810.10527",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "10",
    year = "2018"
}


@article{Carilli:2004nx,
    author = "Carilli, Chris L. and Rawlings, S.",
    title = "{Science with the Square Kilometer Array: Motivation, key science projects, standards and assumptions}",
    eprint = "astro-ph/0409274",
    archivePrefix = "arXiv",
    doi = "10.1016/j.newar.2004.09.001",
    journal = "New Astron. Rev.",
    volume = "48",
    pages = "979",
    year = "2004"
}


@article{Janssen:2014dka,
    author = "Janssen, Gemma and others",
    editor = "Bourke, Tyler L. and others",
    title = "{Gravitational wave astronomy with the SKA}",
    eprint = "1501.00127",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.22323/1.215.0037",
    journal = "PoS",
    volume = "AASKA14",
    pages = "037",
    year = "2015"
}


@article{Weltman:2018zrl,
    author = "Weltman, A. and others",
    title = "{Fundamental physics with the Square Kilometre Array}",
    eprint = "1810.02680",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1017/pasa.2019.42",
    journal = "Publ. Astron. Soc. Austral.",
    volume = "37",
    pages = "e002",
    year = "2020"
}


@article{LISA:2017pwj,
    author = "Amaro-Seoane, Pau and others",
    collaboration = "LISA",
    title = "{Laser Interferometer Space Antenna}",
    eprint = "1702.00786",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "2",
    year = "2017"
}


@article{Baker:2019nia,
    author = "Baker, John and others",
    title = "{The Laser Interferometer Space Antenna: Unveiling the Millihertz Gravitational Wave Sky}",
    eprint = "1907.06482",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "FERMILAB-PUB-19-436-A",
    month = "7",
    year = "2019"
}


@article{Crowder:2005nr,
    author = "Crowder, Jeff and Cornish, Neil J.",
    title = "{Beyond LISA: Exploring future gravitational wave missions}",
    eprint = "gr-qc/0506015",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.72.083005",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "083005",
    year = "2005"
}


@article{Corbin:2005ny,
    author = "Corbin, Vincent and Cornish, Neil J.",
    title = "{Detecting the cosmic gravitational wave background with the big bang observer}",
    eprint = "gr-qc/0512039",
    archivePrefix = "arXiv",
    doi = "10.1088/0264-9381/23/7/014",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "2435--2446",
    year = "2006"
}


@article{Harry:2006fi,
    author = "Harry, G. M. and Fritschel, P. and Shaddock, D. A. and Folkner, W. and Phinney, E. S.",
    title = "{Laser interferometry for the big bang observer}",
    doi = "10.1088/0264-9381/23/15/008",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "4887--4894",
    year = "2006",
    note = "[Erratum: Class.Quant.Grav. 23, 7361 (2006)]"
}


@article{Seto:2001qf,
    author = "Seto, Naoki and Kawamura, Seiji and Nakamura, Takashi",
    title = "{Possibility of direct measurement of the acceleration of the universe using 0.1-Hz band laser interferometer gravitational wave antenna in space}",
    eprint = "astro-ph/0108011",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.87.221103",
    journal = "Phys. Rev. Lett.",
    volume = "87",
    pages = "221103",
    year = "2001"
}


@article{Kawamura:2006up,
    author = "Kawamura, S. and others",
    editor = "Mio, N.",
    title = "{The Japanese space gravitational wave antenna DECIGO}",
    doi = "10.1088/0264-9381/23/8/S17",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "S125--S132",
    year = "2006"
}


@article{Yagi:2011wg,
    author = "Yagi, Kent and Seto, Naoki",
    title = "{Detector configuration of DECIGO/BBO and identification of cosmological neutron-star binaries}",
    eprint = "1101.3940",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.83.044011",
    journal = "Phys. Rev. D",
    volume = "83",
    pages = "044011",
    year = "2011",
    note = "[Erratum: Phys.Rev.D 95, 109901 (2017)]"
}


@article{LIGOScientific:2016wof,
    author = "Abbott, Benjamin P and others",
    collaboration = "LIGO Scientific",
    title = "{Exploring the Sensitivity of Next Generation Gravitational Wave Detectors}",
    eprint = "1607.08697",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "LIGO-P1600143",
    doi = "10.1088/1361-6382/aa51f4",
    journal = "Class. Quant. Grav.",
    volume = "34",
    number = "4",
    pages = "044001",
    year = "2017"
}


@article{Reitze:2019iox,
    author = "Reitze, David and others",
    title = "{Cosmic Explorer: The U.S. Contribution to Gravitational-Wave Astronomy beyond LIGO}",
    eprint = "1907.04833",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "LIGO-P1900316",
    journal = "Bull. Am. Astron. Soc.",
    volume = "51",
    number = "7",
    pages = "035",
    year = "2019"
}


@article{Punturo:2010zz,
    author = "Punturo, M. and others",
    editor = "Ricci, Fulvio",
    title = "{The Einstein Telescope: A third-generation gravitational wave observatory}",
    doi = "10.1088/0264-9381/27/19/194002",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "194002",
    year = "2010"
}


@article{Hild:2010id,
    author = "Hild, S. and others",
    title = "{Sensitivity Studies for Third-Generation Gravitational Wave Observatories}",
    eprint = "1012.0908",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/28/9/094013",
    journal = "Class. Quant. Grav.",
    volume = "28",
    pages = "094013",
    year = "2011"
}


@article{Sathyaprakash:2012jk,
    author = "Sathyaprakash, B. and others",
    editor = "Hannam, Mark and Sutton, Patrick and Hild, Stefan and van den Broeck, Chris",
    title = "{Scientific Objectives of Einstein Telescope}",
    eprint = "1206.0331",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/29/12/124013",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "124013",
    year = "2012",
    note = "[Erratum: Class.Quant.Grav. 30, 079501 (2013)]"
}


@article{Maggiore:2019uih,
    author = "Maggiore, Michele and others",
    title = "{Science Case for the Einstein Telescope}",
    eprint = "1912.02622",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/03/050",
    journal = "JCAP",
    volume = "03",
    pages = "050",
    year = "2020"
}


@article{Harry:2010zz,
    author = "Harry, Gregory M.",
    editor = "Marka, Zsuzsa and Marka, Szabolcs",
    collaboration = "LIGO Scientific",
    title = "{Advanced LIGO: The next generation of gravitational wave detectors}",
    doi = "10.1088/0264-9381/27/8/084006",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "084006",
    year = "2010"
}


@article{LIGOScientific:2014pky,
    author = "Aasi, J. and others",
    collaboration = "LIGO Scientific",
    title = "{Advanced LIGO}",
    eprint = "1411.4547",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/32/7/074001",
    journal = "Class. Quant. Grav.",
    volume = "32",
    pages = "074001",
    year = "2015"
}


@article{VIRGO:2014yos,
    author = "Acernese, F. and others",
    collaboration = "VIRGO",
    title = "{Advanced Virgo: a second-generation interferometric gravitational wave detector}",
    eprint = "1408.3978",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/32/2/024001",
    journal = "Class. Quant. Grav.",
    volume = "32",
    number = "2",
    pages = "024001",
    year = "2015"
}


@article{LIGOScientific:2019lzm,
    author = "Abbott, Rich and others",
    collaboration = "LIGO Scientific, Virgo",
    title = "{Open data from the first and second observing runs of Advanced LIGO and Advanced Virgo}",
    eprint = "1912.11716",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "LIGO-P1900206",
    doi = "10.1016/j.softx.2021.100658",
    journal = "SoftwareX",
    volume = "13",
    pages = "100658",
    year = "2021"
}


@article{Thrane:2013oya,
    author = "Thrane, Eric and Romano, Joseph D.",
    title = "{Sensitivity curves for searches for gravitational-wave backgrounds}",
    eprint = "1310.5300",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1103/PhysRevD.88.124032",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "12",
    pages = "124032",
    year = "2013"
}


@article{Caprini:2015zlo,
    author = "Caprini, Chiara and others",
    title = "{Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions}",
    eprint = "1512.06239",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-15-246",
    doi = "10.1088/1475-7516/2016/04/001",
    journal = "JCAP",
    volume = "04",
    pages = "001",
    year = "2016"
}


@article{Feng:2017vli,
    author = "Feng, Jonathan L. and Galon, Iftah and Kling, Felix and Trojanowski, Sebastian",
    title = "{Dark Higgs bosons at the ForwArd Search ExpeRiment}",
    eprint = "1710.09387",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2017-12",
    doi = "10.1103/PhysRevD.97.055034",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "5",
    pages = "055034",
    year = "2018"
}


@article{FASER:2018eoc,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER\textquoteright{}s physics reach for long-lived particles}",
    eprint = "1811.12522",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2018-19, KYUSHU-RCAPP-2018-06",
    doi = "10.1103/PhysRevD.99.095011",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "9",
    pages = "095011",
    year = "2019"
}


@article{FASER:2018bac,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{Technical Proposal for FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1812.09139",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-LHCC-2018-036, LHCC-P-013, UCI-TR-2018-22, KYUSHU-RCAPP-2018-07",
    month = "12",
    year = "2018"
}


@article{FASER:2019aik,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1901.04468",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2019-01, KYUSHU-RCAPP-2018-08",
    month = "1",
    year = "2019"
}


@article{DUNE:2015lol,
    author = "Acciarri, R. and others",
    collaboration = "DUNE",
    title = "{Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE)}: {Conceptual Design Report, Volume 2: The Physics Program for DUNE at LBNF}",
    eprint = "1512.06148",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-DESIGN-2016-02",
    month = "12",
    year = "2015"
}


@article{Berryman:2019dme,
    author = "Berryman, Jeffrey M. and de Gouvea, Andre and Fox, Patrick J and Kayser, Boris Jules and Kelly, Kevin James and Raaf, Jennifer Lynne",
    title = "{Searches for Decays of New Particles in the DUNE Multi-Purpose Near Detector}",
    eprint = "1912.07622",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-19-607-ND-T, NUHEP-TH/19-16",
    doi = "10.1007/JHEP02(2020)174",
    journal = "JHEP",
    volume = "02",
    pages = "174",
    year = "2020"
}


@article{Batell:2020vqn,
    author = "Batell, Brian and Evans, Jared A. and Gori, Stefania and Rai, Mudit",
    title = "{Dark Scalars and Heavy Neutral Leptons at DarkQuest}",
    eprint = "2008.08108",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2021)049",
    journal = "JHEP",
    volume = "05",
    pages = "049",
    year = "2021"
}


@article{Curtin:2018mvb,
    author = "Curtin, David and others",
    title = "{Long-Lived Particles at the Energy Frontier: The MATHUSLA Physics Case}",
    eprint = "1806.07396",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-264-T",
    doi = "10.1088/1361-6633/ab28d6",
    journal = "Rept. Prog. Phys.",
    volume = "82",
    number = "11",
    pages = "116201",
    year = "2019"
}


@article{Bernardi:1985ny,
    author = "Bernardi, G. and others",
    title = "{Search for Neutrino Decay}",
    reportNumber = "CERN-EP/85-177",
    doi = "10.1016/0370-2693(86)91602-3",
    journal = "Phys. Lett. B",
    volume = "166",
    pages = "479--483",
    year = "1986"
}


@article{Gorbunov:2021ccu,
    author = "Gorbunov, Dmitry and Krasnov, Igor and Suvorov, Sergey",
    title = "{Constraints on light scalars from PS191 results}",
    eprint = "2105.11102",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "INR-TH-2021-012",
    doi = "10.1016/j.physletb.2021.136524",
    journal = "Phys. Lett. B",
    volume = "820",
    pages = "136524",
    year = "2021"
}


@article{SHiP:2015vad,
    author = "Anelli, M. and others",
    collaboration = "SHiP",
    title = "{A facility to Search for Hidden Particles (SHiP) at the CERN SPS}",
    eprint = "1504.04956",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-SPSC-2015-016, SPSC-P-350",
    month = "4",
    year = "2015"
}


@article{Barman:2022njh,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Probing pre-BBN era with Scale Invarint FIMP}",
    eprint = "2203.13269",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-712FT",
    month = "3",
    year = "2022"
}


@article{Barman:2021lot,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Scale invariant FIMP miracle}",
    eprint = "2109.03259",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-698FT",
    doi = "10.1088/1475-7516/2022/03/003",
    journal = "JCAP",
    volume = "03",
    number = "03",
    pages = "003",
    year = "2022"
}

@article{Kost:2021rbi,
    author = "Kost, Jeff and Shin, Chang Sub and Terada, Takahiro",
    title = "{Massless preheating and electroweak vacuum metastability}",
    eprint = "2105.06939",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CTPU-PTC-21-20",
    doi = "10.1103/PhysRevD.105.043508",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "4",
    pages = "043508",
    year = "2022"
}

@article{Ford:1986sy,
    author = "Ford, L. H.",
    title = "{Gravitational Particle Creation and Inflation}",
    reportNumber = "TUTP-86-8",
    doi = "10.1103/PhysRevD.35.2955",
    journal = "Phys. Rev. D",
    volume = "35",
    pages = "2955",
    year = "1987"
}

@article{Chun:2009yu,
    author = "Chun, E. J. and Scopel, S. and Zaballa, I.",
    title = "{Gravitational reheating in quintessential inflation}",
    eprint = "0904.0675",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2009/07/022",
    journal = "JCAP",
    volume = "07",
    pages = "022",
    year = "2009"
}

@article{MoursyXXXX,
    author = "Heurtier, L. and Moursy, A. and Wacquez, L.",
    title = "{To Appear}",
    eprint = "2207.XXXX",
    archivePrefix = "arXiv",
    primaryClass = "hep-th"
}

@article{Campos:2004xw,
    author = "Campos, A. H. and Reis, H. C. and Rosenfeld, R.",
    editor = "Asorey, M. and Shapiro, I. L.",
    title = "{Quintessential inflation and non-oscillatory reheating model}",
    doi = "10.1016/S0920-5632(03)02414-9",
    journal = "Nucl. Phys. B Proc. Suppl.",
    volume = "127",
    pages = "133--137",
    year = "2004"
}



@article{Feng:2002nb,
    author = "Feng, Bo and Li, Ming-zhe",
    title = "{Curvaton reheating in nonoscillatory inflationary models}",
    eprint = "hep-ph/0212213",
    archivePrefix = "arXiv",
    reportNumber = "BIHEP-TH-2002-57",
    doi = "10.1016/S0370-2693(03)00589-6",
    journal = "Phys. Lett. B",
    volume = "564",
    pages = "169--174",
    year = "2003"
}

@article{Dimopoulos:2017zvq,
    author = "Dimopoulos, Konstantinos and Owen, Charlotte",
    title = "{Quintessential Inflation with $\alpha$-attractors}",
    eprint = "1703.00305",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/1475-7516/2017/06/027",
    journal = "JCAP",
    volume = "06",
    pages = "027",
    year = "2017"
}

@article{Okada:2019opp,
    author = "Okada, Nobuchika and Raut, Digesh",
    title = "{Hunting inflatons at FASER}",
    eprint = "1910.09663",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.055022",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "5",
    pages = "055022",
    year = "2021"
}

@article{Arcadi:2021mag,
    author = "Arcadi, Giorgio and Djouadi, Abdelhak and Kado, Marumi",
    title = "{The Higgs-portal for dark matter: effective field theories versus concrete realizations}",
    eprint = "2101.02507",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-021-09411-2",
    journal = "Eur. Phys. J. C",
    volume = "81",
    number = "7",
    pages = "653",
    year = "2021"
}

@article{Heurtier:2017nwl,
    author = "Heurtier, Lucien",
    title = "{The Inflaton Portal to Dark Matter}",
    eprint = "1707.08999",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP12(2017)072",
    journal = "JHEP",
    volume = "12",
    pages = "072",
    year = "2017"
}



==> backup/main_old_v4 <==
@article{Planck:2018vyg,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Buchmuller:2014pla,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Wieck, Clemens",
    title = "{Large-Field Inflation and Supersymmetry Breaking}",
    eprint = "1407.0253",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-14-100, CPHT-RR037.0614",
    doi = "10.1007/JHEP09(2014)053",
    journal = "JHEP",
    volume = "09",
    pages = "053",
    year = "2014"
}


@article{Buchmuller:2015oma,
    author = "Buchmuller, Wilfried and Dudas, Emilian and Heurtier, Lucien and Westphal, Alexander and Wieck, Clemens and Winkler, Martin Wolfgang",
    title = "{Challenges for Large-Field Inflation and Moduli Stabilization}",
    eprint = "1501.05812",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-15-014, CPHT-RR002.0115",
    doi = "10.1007/JHEP04(2015)058",
    journal = "JHEP",
    volume = "04",
    pages = "058",
    year = "2015"
}


@article{Argurio:2017joe,
    author = "Argurio, Riccardo and Coone, Dries and Heurtier, Lucien and Mariotti, Alberto",
    title = "{Sgoldstino-less inflation and low energy SUSY breaking}",
    eprint = "1705.06788",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2017/07/047",
    journal = "JCAP",
    volume = "07",
    pages = "047",
    year = "2017"
}


@article{Heurtier:2019eou,
    author = "Heurtier, Lucien and Huang, Fei",
    title = "{Inflaton portal to a highly decoupled EeV dark matter particle}",
    eprint = "1905.05191",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.100.043507",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "4",
    pages = "043507",
    year = "2019"
}


@article{Enqvist:2016mqj,
    author = "Enqvist, Kari and Karciauskas, Mindaugas and Lebedev, Oleg and Rusak, Stanislav and Zatta, Marco",
    title = "{Postinflationary vacuum instability and Higgs-inflaton couplings}",
    eprint = "1608.08848",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2016/11/025",
    journal = "JCAP",
    volume = "11",
    pages = "025",
    year = "2016"
}


@article{Kost:2021rbi,
    author = "Kost, Jeff and Shin, Chang Sub and Terada, Takahiro",
    title = "{Massless preheating and electroweak vacuum metastability}",
    eprint = "2105.06939",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CTPU-PTC-21-20",
    doi = "10.1103/PhysRevD.105.043508",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "4",
    pages = "043508",
    year = "2022"
}


@article{Akrami:2017cir,
    author = "Akrami, Yashar and Kallosh, Renata and Linde, Andrei and Vardanyan, Valeri",
    title = "{Dark energy, $\alpha$-attractors, and large-scale structure surveys}",
    eprint = "1712.09693",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2018/06/041",
    journal = "JCAP",
    volume = "06",
    pages = "041",
    year = "2018"
}


@article{Dimopoulos:2001ix,
    author = "Dimopoulos, Konstantinos and Valle, J. W. F.",
    title = "{Modeling quintessential inflation}",
    eprint = "astro-ph/0111417",
    archivePrefix = "arXiv",
    reportNumber = "IFIC-01-49, LANCS-01-21-11",
    doi = "10.1016/S0927-6505(02)00115-9",
    journal = "Astropart. Phys.",
    volume = "18",
    pages = "287--306",
    year = "2002"
}


@article{Ellis:2020krl,
    author = "Ellis, John and Nanopoulos, Dimitri V. and Olive, Keith A. and Verner, Sarunas",
    title = "{Non-Oscillatory No-Scale Inflation}",
    eprint = "2008.09099",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMN-TH-3924/20, FTPI-MINN-20/27, KCL-PH-TH/2020-38,
  CERN-TH-2020-123, ACT-05-20, MI-TH-2020",
    doi = "10.1088/1475-7516/2021/03/052",
    journal = "JCAP",
    volume = "03",
    pages = "052",
    year = "2021"
}


@article{Ford:1986sy,
    author = "Ford, L. H.",
    title = "{Gravitational Particle Creation and Inflation}",
    reportNumber = "TUTP-86-8",
    doi = "10.1103/PhysRevD.35.2955",
    journal = "Phys. Rev. D",
    volume = "35",
    pages = "2955",
    year = "1987"
}


@article{Chun:2009yu,
    author = "Chun, E. J. and Scopel, S. and Zaballa, I.",
    title = "{Gravitational reheating in quintessential inflation}",
    eprint = "0904.0675",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2009/07/022",
    journal = "JCAP",
    volume = "07",
    pages = "022",
    year = "2009"
}

@article{MoursyXXXX,
    author = "Heurtier, L. and Moursy, A. and Wacquez, L.",
    title = "{To Appear}",
    eprint = "2207.XXXX",
    archivePrefix = "arXiv",
    primaryClass = "hep-th"
}


@article{Gouttenoire:2021jhk,
    author = "Gouttenoire, Yann and Servant, Geraldine and Simakachorn, Peera",
    title = "{Kination cosmology from scalar fields and gravitational-wave signatures}",
    eprint = "2111.01150",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 21-134",
    month = "11",
    year = "2021"
}


@article{Campos:2004xw,
    author = "Campos, A. H. and Reis, H. C. and Rosenfeld, R.",
    editor = "Asorey, M. and Shapiro, I. L.",
    title = "{Quintessential inflation and non-oscillatory reheating model}",
    doi = "10.1016/S0920-5632(03)02414-9",
    journal = "Nucl. Phys. B Proc. Suppl.",
    volume = "127",
    pages = "133--137",
    year = "2004"
}


@article{Feng:2002nb,
    author = "Feng, Bo and Li, Ming-zhe",
    title = "{Curvaton reheating in nonoscillatory inflationary models}",
    eprint = "hep-ph/0212213",
    archivePrefix = "arXiv",
    reportNumber = "BIHEP-TH-2002-57",
    doi = "10.1016/S0370-2693(03)00589-6",
    journal = "Phys. Lett. B",
    volume = "564",
    pages = "169--174",
    year = "2003"
}


@article{Dimopoulos:2017zvq,
    author = "Dimopoulos, Konstantinos and Owen, Charlotte",
    title = "{Quintessential Inflation with $\alpha$-attractors}",
    eprint = "1703.00305",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/1475-7516/2017/06/027",
    journal = "JCAP",
    volume = "06",
    pages = "027",
    year = "2017"
}


@article{Starobinsky:1985ww,
    author = "Starobinsky, A. A.",
    title = "{Cosmic Background Anisotropy Induced by Isotropic Flat-Spectrum Gravitational-Wave Perturbations}",
    journal = "Sov. Astron. Lett.",
    volume = "11",
    pages = "133",
    year = "1985"
}


@article{Watanabe:2006qe,
    author = "Watanabe, Yuki and Komatsu, Eiichiro",
    title = "{Improved Calculation of the Primordial Gravitational Wave Spectrum in the Standard Model}",
    eprint = "astro-ph/0604176",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.73.123515",
    journal = "Phys. Rev. D",
    volume = "73",
    pages = "123515",
    year = "2006"
}


@article{Saikawa:2018rcs,
    author = "Saikawa, Ken'ichi and Shirai, Satoshi",
    title = "{Primordial gravitational waves, precisely: The role of thermodynamics in the Standard Model}",
    eprint = "1803.01038",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPMU18-0037, MPP-2018-19",
    doi = "10.1088/1475-7516/2018/05/035",
    journal = "JCAP",
    volume = "05",
    pages = "035",
    year = "2018"
}


@article{Bernal:2019lpc,
    author = "Bernal, Nicol\'as and Hajkarim, Fazlollah",
    title = "{Primordial Gravitational Waves in Nonstandard Cosmologies}",
    eprint = "1905.10410",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.100.063502",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "6",
    pages = "063502",
    year = "2019"
}


@article{Weinberg:2003ur,
    author = "Weinberg, Steven",
    title = "{Damping of tensor modes in cosmology}",
    eprint = "astro-ph/0306304",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-02-03",
    doi = "10.1103/PhysRevD.69.023503",
    journal = "Phys. Rev. D",
    volume = "69",
    pages = "023503",
    year = "2004"
}


@article{Drees:2015exa,
    author = "Drees, Manuel and Hajkarim, Fazlollah and Schmitz, Ernany Rossi",
    title = "{The Effects of QCD Equation of State on the Relic Density of WIMP Dark Matter}",
    eprint = "1503.03513",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2015/06/025",
    journal = "JCAP",
    volume = "06",
    pages = "025",
    year = "2015"
}


@article{Aghanim:2018eyx,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Schmitz:2020syl,
    author = "Schmitz, Kai",
    title = "{New Sensitivity Curves for Gravitational-Wave Signals from Cosmological Phase Transitions}",
    eprint = "2002.04615",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-018",
    doi = "10.1007/JHEP01(2021)097",
    journal = "JHEP",
    volume = "01",
    pages = "097",
    year = "2021"
}


@article{McLaughlin:2013ira,
    author = "McLaughlin, Maura A.",
    title = "{The North American Nanohertz Observatory for Gravitational Waves}",
    eprint = "1310.0758",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/0264-9381/30/22/224008",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224008",
    year = "2013"
}


@article{NANOGRAV:2018hou,
    author = "Arzoumanian, Z. and others",
    collaboration = "NANOGRAV",
    title = "{The NANOGrav 11-year Data Set: Pulsar-timing Constraints On The Stochastic Gravitational-wave Background}",
    eprint = "1801.02617",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.HE",
    doi = "10.3847/1538-4357/aabd3b",
    journal = "Astrophys. J.",
    volume = "859",
    number = "1",
    pages = "47",
    year = "2018"
}


@article{Aggarwal:2018mgp,
    author = "Aggarwal, K. and others",
    title = "{The NANOGrav 11-Year Data Set: Limits on Gravitational Waves from Individual Supermassive Black Hole Binaries}",
    eprint = "1812.11585",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.GA",
    doi = "10.3847/1538-4357/ab2236",
    journal = "Astrophys. J.",
    volume = "880",
    pages = "2",
    year = "2019"
}


@article{Brazier:2019mmu,
    author = "Brazier, A. and others",
    title = "{The NANOGrav Program for Gravitational Waves and Fundamental Physics}",
    eprint = "1908.05356",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "8",
    year = "2019"
}


@article{Manchester:2012za,
    author = "Manchester, R. N. and others",
    title = "{The Parkes Pulsar Timing Array Project}",
    eprint = "1210.6130",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1017/pasa.2012.017",
    journal = "Publ. Astron. Soc. Austral.",
    volume = "30",
    pages = "17",
    year = "2013"
}


@article{Shannon:2015ect,
    author = "Shannon, R. M. and others",
    title = "{Gravitational waves from binary supermassive black holes missing in pulsar observations}",
    eprint = "1509.07320",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1126/science.aab1910",
    journal = "Science",
    volume = "349",
    number = "6255",
    pages = "1522--1525",
    year = "2015"
}


@article{Kramer:2013kea,
    author = "Kramer, Michael and Champion, David J.",
    title = "{The European Pulsar Timing Array and the Large European Array for Pulsars}",
    doi = "10.1088/0264-9381/30/22/224009",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224009",
    year = "2013"
}


@article{Lentati:2015qwp,
    author = "Lentati, L. and others",
    title = "{European Pulsar Timing Array Limits On An Isotropic Stochastic Gravitational-Wave Background}",
    eprint = "1504.03692",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stv1538",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "453",
    number = "3",
    pages = "2576--2598",
    year = "2015"
}


@article{Babak:2015lua,
    author = "Babak, Stanislav and others",
    title = "{European Pulsar Timing Array Limits on Continuous Gravitational Waves from Individual Supermassive Black Hole Binaries}",
    eprint = "1509.02165",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stv2092",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "455",
    number = "2",
    pages = "1665--1679",
    year = "2016"
}


@article{Hobbs:2009yy,
    author = "Hobbs, G. and others",
    editor = "Marka, Zsuzsa and Marka, Szabolcs",
    title = "{The international pulsar timing array project: using pulsars as a gravitational wave detector}",
    eprint = "0911.5206",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.SR",
    doi = "10.1088/0264-9381/27/8/084013",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "084013",
    year = "2010"
}


@article{Manchester:2013ndt,
    author = "Manchester, R. N.",
    title = "{The International Pulsar Timing Array}",
    eprint = "1309.7392",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/0264-9381/30/22/224010",
    journal = "Class. Quant. Grav.",
    volume = "30",
    pages = "224010",
    year = "2013"
}


@article{Verbiest:2016vem,
    author = "Verbiest, J. P. W. and others",
    title = "{The International Pulsar Timing Array: First Data Release}",
    eprint = "1602.03640",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1093/mnras/stw347",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "458",
    number = "2",
    pages = "1267--1288",
    year = "2016"
}


@article{Hazboun:2018wpv,
    author = "Hazboun, Jeffrey S. and Mingarelli, Chiara M. F. and Lee, Kejia",
    title = "{The Second International Pulsar Timing Array Mock Data Challenge}",
    eprint = "1810.10527",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "10",
    year = "2018"
}


@article{Carilli:2004nx,
    author = "Carilli, Chris L. and Rawlings, S.",
    title = "{Science with the Square Kilometer Array: Motivation, key science projects, standards and assumptions}",
    eprint = "astro-ph/0409274",
    archivePrefix = "arXiv",
    doi = "10.1016/j.newar.2004.09.001",
    journal = "New Astron. Rev.",
    volume = "48",
    pages = "979",
    year = "2004"
}


@article{Janssen:2014dka,
    author = "Janssen, Gemma and others",
    editor = "Bourke, Tyler L. and others",
    title = "{Gravitational wave astronomy with the SKA}",
    eprint = "1501.00127",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.22323/1.215.0037",
    journal = "PoS",
    volume = "AASKA14",
    pages = "037",
    year = "2015"
}


@article{Weltman:2018zrl,
    author = "Weltman, A. and others",
    title = "{Fundamental physics with the Square Kilometre Array}",
    eprint = "1810.02680",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1017/pasa.2019.42",
    journal = "Publ. Astron. Soc. Austral.",
    volume = "37",
    pages = "e002",
    year = "2020"
}


@article{LISA:2017pwj,
    author = "Amaro-Seoane, Pau and others",
    collaboration = "LISA",
    title = "{Laser Interferometer Space Antenna}",
    eprint = "1702.00786",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "2",
    year = "2017"
}


@article{Baker:2019nia,
    author = "Baker, John and others",
    title = "{The Laser Interferometer Space Antenna: Unveiling the Millihertz Gravitational Wave Sky}",
    eprint = "1907.06482",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "FERMILAB-PUB-19-436-A",
    month = "7",
    year = "2019"
}


@article{Crowder:2005nr,
    author = "Crowder, Jeff and Cornish, Neil J.",
    title = "{Beyond LISA: Exploring future gravitational wave missions}",
    eprint = "gr-qc/0506015",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.72.083005",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "083005",
    year = "2005"
}


@article{Corbin:2005ny,
    author = "Corbin, Vincent and Cornish, Neil J.",
    title = "{Detecting the cosmic gravitational wave background with the big bang observer}",
    eprint = "gr-qc/0512039",
    archivePrefix = "arXiv",
    doi = "10.1088/0264-9381/23/7/014",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "2435--2446",
    year = "2006"
}


@article{Harry:2006fi,
    author = "Harry, G. M. and Fritschel, P. and Shaddock, D. A. and Folkner, W. and Phinney, E. S.",
    title = "{Laser interferometry for the big bang observer}",
    doi = "10.1088/0264-9381/23/15/008",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "4887--4894",
    year = "2006",
    note = "[Erratum: Class.Quant.Grav. 23, 7361 (2006)]"
}


@article{Seto:2001qf,
    author = "Seto, Naoki and Kawamura, Seiji and Nakamura, Takashi",
    title = "{Possibility of direct measurement of the acceleration of the universe using 0.1-Hz band laser interferometer gravitational wave antenna in space}",
    eprint = "astro-ph/0108011",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.87.221103",
    journal = "Phys. Rev. Lett.",
    volume = "87",
    pages = "221103",
    year = "2001"
}


@article{Kawamura:2006up,
    author = "Kawamura, S. and others",
    editor = "Mio, N.",
    title = "{The Japanese space gravitational wave antenna DECIGO}",
    doi = "10.1088/0264-9381/23/8/S17",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "S125--S132",
    year = "2006"
}


@article{Yagi:2011wg,
    author = "Yagi, Kent and Seto, Naoki",
    title = "{Detector configuration of DECIGO/BBO and identification of cosmological neutron-star binaries}",
    eprint = "1101.3940",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.83.044011",
    journal = "Phys. Rev. D",
    volume = "83",
    pages = "044011",
    year = "2011",
    note = "[Erratum: Phys.Rev.D 95, 109901 (2017)]"
}


@article{LIGOScientific:2016wof,
    author = "Abbott, Benjamin P and others",
    collaboration = "LIGO Scientific",
    title = "{Exploring the Sensitivity of Next Generation Gravitational Wave Detectors}",
    eprint = "1607.08697",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "LIGO-P1600143",
    doi = "10.1088/1361-6382/aa51f4",
    journal = "Class. Quant. Grav.",
    volume = "34",
    number = "4",
    pages = "044001",
    year = "2017"
}


@article{Reitze:2019iox,
    author = "Reitze, David and others",
    title = "{Cosmic Explorer: The U.S. Contribution to Gravitational-Wave Astronomy beyond LIGO}",
    eprint = "1907.04833",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "LIGO-P1900316",
    journal = "Bull. Am. Astron. Soc.",
    volume = "51",
    number = "7",
    pages = "035",
    year = "2019"
}


@article{Punturo:2010zz,
    author = "Punturo, M. and others",
    editor = "Ricci, Fulvio",
    title = "{The Einstein Telescope: A third-generation gravitational wave observatory}",
    doi = "10.1088/0264-9381/27/19/194002",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "194002",
    year = "2010"
}


@article{Hild:2010id,
    author = "Hild, S. and others",
    title = "{Sensitivity Studies for Third-Generation Gravitational Wave Observatories}",
    eprint = "1012.0908",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/28/9/094013",
    journal = "Class. Quant. Grav.",
    volume = "28",
    pages = "094013",
    year = "2011"
}


@article{Sathyaprakash:2012jk,
    author = "Sathyaprakash, B. and others",
    editor = "Hannam, Mark and Sutton, Patrick and Hild, Stefan and van den Broeck, Chris",
    title = "{Scientific Objectives of Einstein Telescope}",
    eprint = "1206.0331",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/29/12/124013",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "124013",
    year = "2012",
    note = "[Erratum: Class.Quant.Grav. 30, 079501 (2013)]"
}


@article{Maggiore:2019uih,
    author = "Maggiore, Michele and others",
    title = "{Science Case for the Einstein Telescope}",
    eprint = "1912.02622",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/03/050",
    journal = "JCAP",
    volume = "03",
    pages = "050",
    year = "2020"
}


@article{Harry:2010zz,
    author = "Harry, Gregory M.",
    editor = "Marka, Zsuzsa and Marka, Szabolcs",
    collaboration = "LIGO Scientific",
    title = "{Advanced LIGO: The next generation of gravitational wave detectors}",
    doi = "10.1088/0264-9381/27/8/084006",
    journal = "Class. Quant. Grav.",
    volume = "27",
    pages = "084006",
    year = "2010"
}


@article{LIGOScientific:2014pky,
    author = "Aasi, J. and others",
    collaboration = "LIGO Scientific",
    title = "{Advanced LIGO}",
    eprint = "1411.4547",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/32/7/074001",
    journal = "Class. Quant. Grav.",
    volume = "32",
    pages = "074001",
    year = "2015"
}


@article{VIRGO:2014yos,
    author = "Acernese, F. and others",
    collaboration = "VIRGO",
    title = "{Advanced Virgo: a second-generation interferometric gravitational wave detector}",
    eprint = "1408.3978",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/32/2/024001",
    journal = "Class. Quant. Grav.",
    volume = "32",
    number = "2",
    pages = "024001",
    year = "2015"
}


@article{LIGOScientific:2019lzm,
    author = "Abbott, Rich and others",
    collaboration = "LIGO Scientific, Virgo",
    title = "{Open data from the first and second observing runs of Advanced LIGO and Advanced Virgo}",
    eprint = "1912.11716",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "LIGO-P1900206",
    doi = "10.1016/j.softx.2021.100658",
    journal = "SoftwareX",
    volume = "13",
    pages = "100658",
    year = "2021"
}


@article{Thrane:2013oya,
    author = "Thrane, Eric and Romano, Joseph D.",
    title = "{Sensitivity curves for searches for gravitational-wave backgrounds}",
    eprint = "1310.5300",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1103/PhysRevD.88.124032",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "12",
    pages = "124032",
    year = "2013"
}


@article{Caprini:2015zlo,
    author = "Caprini, Chiara and others",
    title = "{Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions}",
    eprint = "1512.06239",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-15-246",
    doi = "10.1088/1475-7516/2016/04/001",
    journal = "JCAP",
    volume = "04",
    pages = "001",
    year = "2016"
}


@article{Feng:2017vli,
    author = "Feng, Jonathan L. and Galon, Iftah and Kling, Felix and Trojanowski, Sebastian",
    title = "{Dark Higgs bosons at the ForwArd Search ExpeRiment}",
    eprint = "1710.09387",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2017-12",
    doi = "10.1103/PhysRevD.97.055034",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "5",
    pages = "055034",
    year = "2018"
}


@article{FASER:2018eoc,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER\textquoteright{}s physics reach for long-lived particles}",
    eprint = "1811.12522",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UCI-TR-2018-19, KYUSHU-RCAPP-2018-06",
    doi = "10.1103/PhysRevD.99.095011",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "9",
    pages = "095011",
    year = "2019"
}


@article{FASER:2018bac,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{Technical Proposal for FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1812.09139",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-LHCC-2018-036, LHCC-P-013, UCI-TR-2018-22, KYUSHU-RCAPP-2018-07",
    month = "12",
    year = "2018"
}


@article{FASER:2019aik,
    author = "Ariga, Akitaka and others",
    collaboration = "FASER",
    title = "{FASER: ForwArd Search ExpeRiment at the LHC}",
    eprint = "1901.04468",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2019-01, KYUSHU-RCAPP-2018-08",
    month = "1",
    year = "2019"
}


@article{DUNE:2015lol,
    author = "Acciarri, R. and others",
    collaboration = "DUNE",
    title = "{Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE)}: {Conceptual Design Report, Volume 2: The Physics Program for DUNE at LBNF}",
    eprint = "1512.06148",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-DESIGN-2016-02",
    month = "12",
    year = "2015"
}


@article{Berryman:2019dme,
    author = "Berryman, Jeffrey M. and de Gouvea, Andre and Fox, Patrick J and Kayser, Boris Jules and Kelly, Kevin James and Raaf, Jennifer Lynne",
    title = "{Searches for Decays of New Particles in the DUNE Multi-Purpose Near Detector}",
    eprint = "1912.07622",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-19-607-ND-T, NUHEP-TH/19-16",
    doi = "10.1007/JHEP02(2020)174",
    journal = "JHEP",
    volume = "02",
    pages = "174",
    year = "2020"
}


@article{Batell:2020vqn,
    author = "Batell, Brian and Evans, Jared A. and Gori, Stefania and Rai, Mudit",
    title = "{Dark Scalars and Heavy Neutral Leptons at DarkQuest}",
    eprint = "2008.08108",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2021)049",
    journal = "JHEP",
    volume = "05",
    pages = "049",
    year = "2021"
}


@article{Curtin:2018mvb,
    author = "Curtin, David and others",
    title = "{Long-Lived Particles at the Energy Frontier: The MATHUSLA Physics Case}",
    eprint = "1806.07396",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-264-T",
    doi = "10.1088/1361-6633/ab28d6",
    journal = "Rept. Prog. Phys.",
    volume = "82",
    number = "11",
    pages = "116201",
    year = "2019"
}


@article{Bernardi:1985ny,
    author = "Bernardi, G. and others",
    title = "{Search for Neutrino Decay}",
    reportNumber = "CERN-EP/85-177",
    doi = "10.1016/0370-2693(86)91602-3",
    journal = "Phys. Lett. B",
    volume = "166",
    pages = "479--483",
    year = "1986"
}


@article{Gorbunov:2021ccu,
    author = "Gorbunov, Dmitry and Krasnov, Igor and Suvorov, Sergey",
    title = "{Constraints on light scalars from PS191 results}",
    eprint = "2105.11102",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "INR-TH-2021-012",
    doi = "10.1016/j.physletb.2021.136524",
    journal = "Phys. Lett. B",
    volume = "820",
    pages = "136524",
    year = "2021"
}


@article{SHiP:2015vad,
    author = "Anelli, M. and others",
    collaboration = "SHiP",
    title = "{A facility to Search for Hidden Particles (SHiP) at the CERN SPS}",
    eprint = "1504.04956",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-SPSC-2015-016, SPSC-P-350",
    month = "4",
    year = "2015"
}


@article{Okada:2019opp,
    author = "Okada, Nobuchika and Raut, Digesh",
    title = "{Hunting inflatons at FASER}",
    eprint = "1910.09663",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.055022",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "5",
    pages = "055022",
    year = "2021"
}


@article{Arcadi:2021mag,
    author = "Arcadi, Giorgio and Djouadi, Abdelhak and Kado, Marumi",
    title = "{The Higgs-portal for dark matter: effective field theories versus concrete realizations}",
    eprint = "2101.02507",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-021-09411-2",
    journal = "Eur. Phys. J. C",
    volume = "81",
    number = "7",
    pages = "653",
    year = "2021"
}


@article{Barman:2022njh,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Probing pre-BBN era with Scale Invarint FIMP}",
    eprint = "2203.13269",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-712FT",
    month = "3",
    year = "2022"
}


@article{Barman:2021lot,
    author = "Barman, Basabendu and Ghoshal, Anish",
    title = "{Scale invariant FIMP miracle}",
    eprint = "2109.03259",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PI/UAN-2021-698FT",
    doi = "10.1088/1475-7516/2022/03/003",
    journal = "JCAP",
    volume = "03",
    number = "03",
    pages = "003",
    year = "2022"
}


@article{Dasgupta:2022isg,
    author = "Dasgupta, Arnab and Dev, P. S. Bhupal and Ghoshal, Anish and Mazumdar, Anupam",
    title = "{Gravitational Wave Pathway to Testable Leptogenesis}",
    eprint = "2206.07032",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2022"
}


@article{Bhaumik:2022pil,
    author = "Bhaumik, Nilanjandev and Ghoshal, Anish and Lewicki, Marek",
    title = "{Doubly peaked induced stochastic gravitational wave background : Testing baryogenesis from primordial black holes}",
    eprint = "2205.06260",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    month = "5",
    year = "2022"
}


@article{Barman:2022yos,
    author = "Barman, Basabendu and Borah, Debasish and Dasgupta, Arnab and Ghoshal, Anish",
    title = "{Probing high scale Dirac leptogenesis via gravitational waves from domain walls}",
    eprint = "2205.03422",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.106.015007",
    journal = "Phys. Rev. D",
    volume = "106",
    number = "1",
    pages = "015007",
    year = "2022"
}


@article{Ghoshal:2022jdt,
    author = "Ghoshal, Anish and Saha, Pankaj",
    title = "{Detectable Gravitational Waves from (P)-reheating probes non-thermal Dark Matter}",
    eprint = "2203.14424",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@article{Dunsky:2021tih,
    author = "Dunsky, David I. and Ghoshal, Anish and Murayama, Hitoshi and Sakakihara, Yuki and White, Graham",
    title = "{Gravitational Wave Gastronomy}",
    eprint = "2111.08750",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "11",
    year = "2021"
}


@article{Bernal:2020ywq,
    author = "Bernal, Nicol\'as and Ghoshal, Anish and Hajkarim, Fazlollah and Lambiase, Gaetano",
    title = "{Primordial Gravitational Wave Signals in Modified Cosmologies}",
    eprint = "2008.04959",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/1475-7516/2020/11/051",
    journal = "JCAP",
    volume = "11",
    pages = "051",
    year = "2020"
}


@article{Ghoshal:2020vud,
    author = "Ghoshal, Anish and Salvio, Alberto",
    title = "{Gravitational waves from fundamental axion dynamics}",
    eprint = "2007.00005",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP12(2020)049",
    journal = "JHEP",
    volume = "12",
    pages = "049",
    year = "2020"
}


@article{Heurtier:2017nwl,
    author = "Heurtier, Lucien",
    title = "{The Inflaton Portal to Dark Matter}",
    eprint = "1707.08999",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP12(2017)072",
    journal = "JHEP",
    volume = "12",
    pages = "072",
    year = "2017"
}


==> backup/ref_old <==
\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{1}


%\begin{thebibliography}{99}

%%\cite{Haber:1984rc}
%\bibitem{Haber:1984rc}
%H.~E.~Haber and G.~L.~Kane,
%%``The Search for Supersymmetry: Probing Physics Beyond the Standard Model,''
%Phys. Rept. \textbf{117}, 75-263 (1985)
%doi:10.1016/0370-1573(85)90051-1
%%5159 citations counted in INSPIRE as of 18 Nov 2020


%%\cite{Ostrogradsky:1850fid}
%\bibitem{Ostrogradsky:1850fid}
%M.~Ostrogradsky,
%%``M\'emoires sur les \'equations diff\'erentielles, relatives au probl\`eme des isop\'erim\`etres,''
%Mem. Acad. St. Petersbourg \textbf{6}, no.4, 385-517 (1850)
%%87 citations counted in INSPIRE as of 20 Nov 2020

%\cite{Moffat:1990jj}
%\bibitem{Moffat:1990jj}
%J.~W.~Moffat,
%%``Finite nonlocal gauge field theory,''
%Phys. Rev. D \textbf{41}, 1177-1184 (1990)
%doi:10.1103/PhysRevD.41.1177
%%100 citations counted in INSPIRE as of 18 Nov 2020

%%\cite{Evens:1990wf}
%\bibitem{Evens:1990wf}
%D.~Evens, J.~W.~Moffat, G.~Kleppe and R.~P.~Woodard,
%%``Nonlocal regularizations of gauge theories,''
%Phys. Rev. D \textbf{43}, no.2, 499-519 (1991)
%doi:10.1103/PhysRevD.43.499
%%140 citations counted in INSPIRE as of 18 Nov 2020


%\bibitem{Tomboulis:2015gfa} 
%E.~T.~Tomboulis,
%%``Nonlocal and quasilocal field theories,''
%Phys.\ Rev.\ D {\bf 92}, no. 12, 125037 (2015)
%%  doi:10.1103/PhysRevD.92.125037
%[arXiv:1507.00981 [hep-th]].
%%%CITATION = doi:10.1103/PhysRevD.92.125037;%%
%%53 citations counted in INSPIRE as of 06 Jul 2018

%%\cite{Moffat:2011an}
%\bibitem{Moffat:2011an}
%J.~W.~Moffat,
%%``Ultraviolet Complete Quantum Field Theory and Gauge Invariance,''
%[arXiv:1104.5706 [hep-th]].
%%9 citations counted in INSPIRE as of 26 Oct 2020

%\cite{Taylor:2003gn}
\bibitem{Taylor:2003gn}
W.~Taylor and B.~Zwiebach,
%``D-branes, tachyons, and string field theory,''
TASI 2001
[arXiv:hep-th/0311017 [hep-th]].

%\cite{Moffat:1990jj}
\bibitem{Moffat:1990jj}
J.~W.~Moffat,
%``Finite nonlocal gauge field theory,''
Phys. Rev. D \textbf{41}, 1177-1184 (1990)
doi:10.1103/PhysRevD.41.1177
%100 citations counted in INSPIRE as of 18 Nov 2020

%\cite{Evens:1990wf}
\bibitem{Evens:1990wf}
D.~Evens, J.~W.~Moffat, G.~Kleppe and R.~P.~Woodard,
%``Nonlocal regularizations of gauge theories,''
Phys. Rev. D \textbf{43}, no.2, 499-519 (1991)
doi:10.1103/PhysRevD.43.499
%140 citations counted in INSPIRE as of 18 Nov 2020

\bibitem{Tomboulis:1997gg} 
E.~T.~Tomboulis, 
%"Superrenormalizable gauge and gravitational theories,"
hep-th/9702146.

%\cite{Moffat:2011an}
\bibitem{Moffat:2011an}
J.~W.~Moffat,
%``Ultraviolet Complete Quantum Field Theory and Gauge Invariance,''
[arXiv:1104.5706 [hep-th]].
%9 citations counted in INSPIRE as of 26 Oct 2020

\bibitem{Tomboulis:2015gfa} 
E.~T.~Tomboulis,
%``Nonlocal and quasilocal field theories,''
Phys.\ Rev.\ D {\bf 92}, no. 12, 125037 (2015)
%  doi:10.1103/PhysRevD.92.125037
[arXiv:1507.00981 [hep-th]].
%%CITATION = doi:10.1103/PhysRevD.92.125037;%%
%53 citations counted in INSPIRE as of 06 Jul 2018

%\cite{Kleppe:1991rv}
\bibitem{Kleppe:1991rv}
G.~Kleppe and R.~P.~Woodard,
%``Nonlocal Yang-Mills,''
Nucl. Phys. B \textbf{388}, 81-112 (1992)
doi:10.1016/0550-3213(92)90546-N
[arXiv:hep-th/9203016 [hep-th]].
%70 citations counted in INSPIRE as of 10 Jan 2021





\bibitem{sft1}
E.~Witten, 
%``{Noncommutative Geometry and String Field Theory},'' 
{\em Nucl.Phys.}~B268, p.~253, 1986.

\bibitem{sft2}
V.~A. Kostelecky and S.~Samuel,
%``{On a Nonperturbative Vacuum for the Open
%  Bosonic String},'' 
{\em Nucl.Phys.}~B336, p.~263, 1990.

\bibitem{sft3}
V.~A. Kostelecky and S.~Samuel, 
%``{The Static Tachyon Potential in the Open
%  Bosonic String Theory},'' 
{\em Phys.Lett.}, vol.~B207, p.~169, 1988.

\bibitem{padic1}
P.~G. Freund and M.~Olson, 
%``{NONARCHIMEDEAN STRINGS},'' 
{\em Phys.Lett.}~B199, p.~186, 1987.

\bibitem{padic2}
P.~G. Freund and E.~Witten, 
%``{ADELIC STRING AMPLITUDES},'' 
{\em Phys.Lett.} B199, p.~191, 1987.

\bibitem{padic3}
L.~Brekke, P.~G. Freund, M.~Olson, and E.~Witten, 
%``{Nonarchimedean String
%  Dynamics},'' 
{\em Nucl.Phys.}~B302, p.~365, 1988.

\bibitem{Frampton-padic}
P.~H. Frampton and Y.~Okada, 
%``{Effective Scalar Field Theory of $P^-$adic
%  String},''
 {\em Phys.Rev.}, vol.~D37, pp.~3077--3079, 1988.

\bibitem{marc}
T.~Biswas, M.~Grisaru, and W.~Siegel, 
%``{Linear Regge trajectories from
%  worldsheet lattice parton field theory},'' 
  {\em Nucl.Phys.}, vol.~B708,
  pp.~317--344, 2005.

\bibitem{Tseytlin:1995uq} 
  A.~A.~Tseytlin,
  %``On singularities of spherically symmetric backgrounds in string theory,''
  Phys.\ Lett.\ B {\bf 363}, 223 (1995)
 % doi:10.1016/0370-2693(95)01228-7
 % [hep-th/9509050].
  %%CITATION = doi:10.1016/0370-2693(95)01228-7;%%
  %60 citations counted in INSPIRE as of 17 Jul 2017
  
\bibitem{Siegel:2003vt} 
  W.~Siegel,
%  ``Stringy gravity at short distances,''
  hep-th/0309093.
  %%CITATION = HEP-TH/0309093;%%
  %30 citations counted in INSPIRE as of 17 Jul 2017
  


%\bibitem{sft1}
%E.~Witten, 
%%``{Noncommutative Geometry and String Field Theory},'' 
%{\em Nucl.Phys.}~B268, p.~253, 1986.
%
%\bibitem{sft2}
%V.~A. Kostelecky and S.~Samuel,
%%``{On a Nonperturbative Vacuum for the Open
%%  Bosonic String},'' 
%{\em Nucl.Phys.}~B336, p.~263, 1990.
%
%\bibitem{sft3}
%V.~A. Kostelecky and S.~Samuel, 
%%``{The Static Tachyon Potential in the Open
%%  Bosonic String Theory},'' 
%{\em Phys.Lett.}, vol.~B207, p.~169, 1988.
%
%\bibitem{padic1}
%P.~G. Freund and M.~Olson, 
%%``{NONARCHIMEDEAN STRINGS},'' 
%{\em Phys.Lett.}~B199, p.~186, 1987.
%
%\bibitem{padic2}
%P.~G. Freund and E.~Witten, 
%%``{ADELIC STRING AMPLITUDES},'' 
%{\em Phys.Lett.} B199, p.~191, 1987.
%
%\bibitem{padic3}
%L.~Brekke, P.~G. Freund, M.~Olson, and E.~Witten, 
%%``{Nonarchimedean String
%%  Dynamics},'' 
%{\em Nucl.Phys.}~B302, p.~365, 1988.
%
%\bibitem{Frampton-padic}
%P.~H. Frampton and Y.~Okada, 
%%``{Effective Scalar Field Theory of $P^-$adic
%%  String},''
 %{\em Phys.Rev.}, vol.~D37, pp.~3077--3079, 1988.
%
%\bibitem{marc}
%T.~Biswas, M.~Grisaru, and W.~Siegel, 
%%``{Linear Regge trajectories from
%%  worldsheet lattice parton field theory},'' 
  %{\em Nucl.Phys.}, vol.~B708,
  %pp.~317--344, 2005.
%
%\bibitem{Tseytlin:1995uq} 
  %A.~A.~Tseytlin,
  %%``On singularities of spherically symmetric backgrounds in string theory,''
  %Phys.\ Lett.\ B {\bf 363}, 223 (1995)
 %% doi:10.1016/0370-2693(95)01228-7
 %% [hep-th/9509050].
  %%%CITATION = doi:10.1016/0370-2693(95)01228-7;%%
  %%60 citations counted in INSPIRE as of 17 Jul 2017
  %
%\bibitem{Siegel:2003vt} 
  %W.~Siegel,
%%  ``Stringy gravity at short distances,''
  %hep-th/0309093.
  %%%CITATION = HEP-TH/0309093;%%
  %%30 citations counted in INSPIRE as of 17 Jul 2017

%\cite{Calcagni:2013eua}
\bibitem{Calcagni:2013eua}
G.~Calcagni and L.~Modesto,
%``Nonlocality in string theory,''
J. Phys. A \textbf{47}, no.35, 355402 (2014)
doi:10.1088/1751-8113/47/35/355402
[arXiv:1310.4957 [hep-th]].
%%45 citations counted in INSPIRE as of 26 Oct 2020

%\cite{Modesto:2011kw}
\bibitem{Modesto:2011kw}
L.~Modesto,
%``Super-renormalizable Quantum Gravity,''
Phys. Rev. D \textbf{86}, 044005 (2012)
doi:10.1103/PhysRevD.86.044005
[arXiv:1107.2403 [hep-th]].
%352 citations counted in INSPIRE as of 10 Jan 2021

%\cite{Modesto:2012ga}
\bibitem{Modesto:2012ga}
L.~Modesto,
%``Super-renormalizable Higher-Derivative Quantum Gravity,''
[arXiv:1202.0008 [hep-th]].
%38 citations counted in INSPIRE as of 10 Jan 2021

%\cite{Modesto:2015foa}
\bibitem{Modesto:2015foa}
L.~Modesto, M.~Piva and L.~Rachwal,
%``Finite quantum gauge theories,''
Phys. Rev. D \textbf{94}, no.2, 025021 (2016)
doi:10.1103/PhysRevD.94.025021
[arXiv:1506.06227 [hep-th]].
%31 citations counted in INSPIRE as of 10 Jan 2021

%\cite{Modesto:2017hzl}
\bibitem{Modesto:2017hzl}
L.~Modesto, L.~Rachwa\l{} and I.~L.~Shapiro,
%``Renormalization group in super-renormalizable quantum gravity,''
Eur. Phys. J. C \textbf{78}, no.7, 555 (2018)
doi:10.1140/epjc/s10052-018-6035-2
[arXiv:1704.03988 [hep-th]].
%25 citations counted in INSPIRE as of 10 Jan 2021



%\cite{Haber:1984rc}
\bibitem{Haber:1984rc}
H.~E.~Haber and G.~L.~Kane,
%``The Search for Supersymmetry: Probing Physics Beyond the Standard Model,''
Phys. Rept. \textbf{117}, 75-263 (1985)
doi:10.1016/0370-1573(85)90051-1
%5159 citations counted in INSPIRE as of 18 Nov 2020



%\cite{Krasnikov:1987yj}
\bibitem{Krasnikov:1987yj}
N.~V.~Krasnikov,
%``NONLOCAL GAUGE THEORIES,''
Theor. Math. Phys. \textbf{73}, 1184-1190 (1987)
doi:10.1007/BF01017588
%86 citations counted in INSPIRE as of 08 Mar 2021
  
  %\cite{Biswas:2014yia}
\bibitem{Biswas:2014yia} 
  T.~Biswas and N.~Okada,
  %``Towards LHC physics with nonlocal Standard Model,''
  Nucl.\ Phys.\ B {\bf 898}, 113 (2015)
  doi:10.1016/j.nuclphysb.2015.06.023
  [arXiv:1407.3331 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2015.06.023;%%
  %37 citations counted in INSPIRE as of 23 Sep 2018
  
  %\cite{Ghoshal:2017egr}
\bibitem{Ghoshal:2017egr} 
  A.~Ghoshal, A.~Mazumdar, N.~Okada and D.~Villalba,
  %``Stability of infinite derivative Abelian Higgs models,''
  Phys.\ Rev.\ D {\bf 97}, no. 7, 076011 (2018)
  doi:10.1103/PhysRevD.97.076011
  [arXiv:1709.09222 [hep-th]].
  %%CITATION = doi:10.1103/PhysRevD.97.076011;%%
  %8 citations counted in INSPIRE as of 23 Sep 2018
  
  %\cite{Buoninfante:2018mre}
\bibitem{Buoninfante:2018mre}
L.~Buoninfante, G.~Lambiase and A.~Mazumdar,
%``Ghost-free infinite derivative quantum field theory,''
Nucl. Phys. B \textbf{944}, 114646 (2019)
doi:10.1016/j.nuclphysb.2019.114646
[arXiv:1805.03559 [hep-th]].
%49 citations counted in INSPIRE as of 18 Nov 2020


\bibitem{Olive:2016xmw} 
  C.~Patrignani {\it et al.} [Particle Data Group],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 40}, no. 10, 100001 (2016).

%\cite{Ghoshal:2018gpq} 
\bibitem{Ghoshal:2018gpq}
A.~Ghoshal,
%``Scalar dark matter probes the scale of nonlocality,''
Int. J. Mod. Phys. A \textbf{34}, no.24, 1950130 (2019)
doi:10.1142/S0217751X19501306
[arXiv:1812.02314 [hep-ph]].
%4 citations counted in INSPIRE as of 06 Mar 2021

%\cite{Buoninfante:2018gce}
\bibitem{Buoninfante:2018gce}
L.~Buoninfante, A.~Ghoshal, G.~Lambiase and A.~Mazumdar,
%``Transmutation of nonlocal scale in infinite derivative field theories,''
Phys. Rev. D \textbf{99}, no.4, 044032 (2019)
doi:10.1103/PhysRevD.99.044032
[arXiv:1812.01441 [hep-th]].
%20 citations counted in INSPIRE as of 06 Mar 2021
  
  %\cite{Ghoshal:2020lfd} Ghoshal:2017egr
\bibitem{Ghoshal:2020lfd}
A.~Ghoshal, A.~Mazumdar, N.~Okada and D.~Villalba,
%``Non-local Non-Abelian Gauge Theory: Conformal Invariance and $\beta$-function,''
[arXiv:2010.15919 [hep-ph]].
%0 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Frasca:2020jbe}
\bibitem{Frasca:2020jbe}
M.~Frasca and A.~Ghoshal,
%``Mass Gap in Infinite Derivative Non-local Higgs: Dyson-Schwinger Approach,''
[arXiv:2011.10586 [hep-th]].
%0 citations counted in INSPIRE as of 13 Dec 2020


%\cite{Frasca:2021guf}
\bibitem{Frasca:2021guf}
M.~Frasca and A.~Ghoshal,
%``Strongly Coupled String-inspired Infinite Derivative Non-local Yang-Mills: Diluted Mass Gap and Conformal Invariance,''
[arXiv:2102.10665 [hep-th]].
%0 citations counted in INSPIRE as of 07 Mar 2021

%\cite{Frasca:2021iip}
\bibitem{Frasca:2021iip}
M.~Frasca, A.~Ghoshal and N.~Okada,
%``Confinement and Renormalization Group Equations in String-inspired Non-local Gauge Theories,''
[arXiv:2106.07629 [hep-th]].
%0 citations counted in INSPIRE as of 22 Jun 2021

%\cite{Boos:2021chb}
\bibitem{Boos:2021chb}
J.~Boos and C.~D.~Carone,
%``Asymptotic nonlocality,''
[arXiv:2104.11195 [hep-th]].
%1 citations counted in INSPIRE as of 15 Jun 2021



%%%%% RG papers (taken from Litim and Sannino paper) %%%%%%%%%
  
%\cite{Wilson:1971bg}
\bibitem{Wilson:1971bg}
K.~G.~Wilson,
%``Renormalization group and critical phenomena. 1. Renormalization group and the Kadanoff scaling picture,''
Phys. Rev. B \textbf{4}, 3174-3183 (1971)
doi:10.1103/PhysRevB.4.3174
%779 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Wilson:1971dh}
\bibitem{Wilson:1971dh}
K.~G.~Wilson,
%``Renormalization group and critical phenomena. 2. Phase space cell analysis of critical behavior,''
Phys. Rev. B \textbf{4}, 3184-3205 (1971)
doi:10.1103/PhysRevB.4.3184
%637 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Gross:1973id}
\bibitem{Gross:1973id}
D.~J.~Gross and F.~Wilczek,
%``Ultraviolet Behavior of Nonabelian Gauge Theories,''
Phys. Rev. Lett. \textbf{30}, 1343-1346 (1973)
doi:10.1103/PhysRevLett.30.1343
%5438 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Politzer:1973fx}
\bibitem{Politzer:1973fx}
H.~D.~Politzer,
%``Reliable Perturbative Results for Strong Interactions?,''
Phys. Rev. Lett. \textbf{30}, 1346-1349 (1973)
doi:10.1103/PhysRevLett.30.1346
%5244 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Callaway:1988ya}
\bibitem{Callaway:1988ya}
D.~J.~E.~Callaway,
%``Triviality Pursuit: Can Elementary Scalar Particles Exist?,''
Phys. Rept. \textbf{167}, 241 (1988)
doi:10.1016/0370-1573(88)90008-7
%227 citations counted in INSPIRE as of 30 Jan 2021
\bibitem{Weinberg:1980gg} S. Weinberg, (1979), in General Relativity: An Einstein centenary survey, ed. S. W. Hawking and W. Israel, 790--831.
%\cite{Litim:2011cp}
\bibitem{Litim:2011cp}
D.~F.~Litim,
%``Renormalisation group and the Planck scale,''
Phil. Trans. Roy. Soc. Lond. A \textbf{369}, 2759-2778 (2011)
doi:10.1098/rsta.2011.0103
[arXiv:1102.4624 [hep-th]].
%181 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Litim:2006dx}
\bibitem{Litim:2006dx}
D.~F.~Litim,
%``On fixed points of quantum gravity,''
AIP Conf. Proc. \textbf{841}, no.1, 322-329 (2006)
doi:10.1063/1.2218188
[arXiv:hep-th/0606044 [hep-th]].
%85 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Niedermaier:2006ns}
\bibitem{Niedermaier:2006ns}
M.~Niedermaier,
%``The Asymptotic safety scenario in quantum gravity: An Introduction,''
Class. Quant. Grav. \textbf{24}, R171-230 (2007)
doi:10.1088/0264-9381/24/18/R01
[arXiv:gr-qc/0610018 [gr-qc]].
%239 citations counted in INSPIRE as of 30 Jan 2021
\bibitem{Niedermaier:2006wt}
Niedermaier, M., Reuter, M. The Asymptotic Safety Scenario in Quantum Gravity. Living Rev. Relativ. 9, 5 (2006). https://doi.org/10.12942/lrr-2006-5
%\cite{Percacci:2007sz}
\bibitem{Percacci:2007sz}
R.~Percacci,
%``Asymptotic Safety,''
[arXiv:0709.3851 [hep-th]].
%265 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Litim:2008tt}
\bibitem{Litim:2008tt}
D.~F.~Litim,
%``Fixed Points of Quantum Gravity and the Renormalisation Group,''
PoS \textbf{QG-Ph}, 024 (2007)
doi:10.22323/1.043.0024
[arXiv:0810.3675 [hep-th]].
%138 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Reuter:2012id}
\bibitem{Reuter:2012id}
M.~Reuter and F.~Saueressig,
%``Quantum Einstein Gravity,''
New J. Phys. \textbf{14}, 055022 (2012)
doi:10.1088/1367-2630/14/5/055022
[arXiv:1202.2274 [hep-th]].
%321 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Litim:2014uca}
\bibitem{Litim:2014uca}
D.~F.~Litim and F.~Sannino,
%``Asymptotic safety guaranteed,''
JHEP \textbf{12}, 178 (2014)
doi:10.1007/JHEP12(2014)178
[arXiv:1406.2337 [hep-th]].
%192 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Giudice:2014tma}
\bibitem{Giudice:2014tma}
G.~F.~Giudice, G.~Isidori, A.~Salvio and A.~Strumia,
%``Softened Gravity and the Extension of the Standard Model up to Infinite Energy,''
JHEP \textbf{02}, 137 (2015)
doi:10.1007/JHEP02(2015)137
[arXiv:1412.2769 [hep-ph]].
%87 citations counted in INSPIRE as of 30 Jan 2021
%\cite{Pelaggi:2017abg}
\bibitem{Pelaggi:2017abg}
G.~M.~Pelaggi, A.~D.~Plascencia, A.~Salvio, F.~Sannino, J.~Smirnov and A.~Strumia,
%``Asymptotically Safe Standard Model Extensions?,''
Phys. Rev. D \textbf{97}, no.9, 095013 (2018)
doi:10.1103/PhysRevD.97.095013
[arXiv:1708.00437 [hep-ph]].
%58 citations counted in INSPIRE as of 30 Jan 2021
%%%%%

%\cite{Kogut:2004su}
\bibitem{Kogut:2004su} 
  J.~B.~Kogut and M.~A.~Stephanov,
  ``The phases of quantum chromodynamics: From confinement to extreme environments,''
  %Camb.\ Monogr.\ Part.\ Phys.\ Nucl.\ Phys.\ Cosmol.\  {\bf 21}, 1 (2004).
	(Cambridge University Press, Cambridge, 2004).
  %%CITATION = CMPCE,21,1;%%
  %33 citations counted in INSPIRE as of 08 Sep 2017
	
\cite{Kugo:1977zq}
\bibitem{Kugo:1977zq} 
 T.~Kugo and I.~Ojima,
 %``Manifestly Covariant Canonical Formulation of Yang--Mills Field Theories: Physical State Subsidiary Conditions and Physical S Matrix Unitarity,''
 Phys.\ Lett.\  {\bf 73B}, 459 (1978).
 %doi:10.1016/0370-2693(78)90765-7
 %%CITATION = doi:10.1016/0370-2693(78)90765-7;%%
 %266 citations counted in INSPIRE as of 28 Apr 2017
	
%\cite{Kugo:1979gm}
\bibitem{Kugo:1979gm} 
 T.~Kugo and I.~Ojima,
 %``Local Covariant Operator Formalism of Nonabelian Gauge Theories and Quark Confinement Problem,''
 Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 66}, 1 (1979).
 %doi:10.1143/PTPS.66.1
 %%CITATION = doi:10.1143/PTPS.66.1;%%
 %917 citations counted in INSPIRE as of 28 Apr 2017
	
%\cite{Nishijima:1993fq}
\bibitem{Nishijima:1993fq} 
  K.~Nishijima,
  %``Confinement of quarks and gluons,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 9}, 3799 (1994).
  %doi:10.1142/S0217751X94001539
  %%CITATION = doi:10.1142/S0217751X94001539;%%
  %28 citations counted in INSPIRE as of 18 Apr 2017
	
%\cite{Nishijima:1995ie}
\bibitem{Nishijima:1995ie} 
  K.~Nishijima,
  %``Confinement of quarks and gluons. 2,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 10}, 3155 (1995).
  %doi:10.1142/S0217751X95001510
  %%CITATION = doi:10.1142/S0217751X95001510;%%
  %21 citations counted in INSPIRE as of 18 Apr 2017
	
%%\cite{Nishijima:1996ji}
%\bibitem{Nishijima:1996ji} 
%  K.~Nishijima,
%  %``BRS invariance, asymptotic freedom and colour confinement. (A review),''
%  Czech.\ J.\ Phys.\  {\bf 46}, 1 (1996).
%  %doi:10.1007/BF01692238
%  %%CITATION = doi:10.1007/BF01692238;%%
%  %48 citations counted in INSPIRE as of 18 Apr 2017
	
%\cite{Chaichian:2000sf}
\bibitem{Chaichian:2000sf} 
  M.~Chaichian and K.~Nishijima,
  %``Renormalization constant of the colour gauge field as a probe of confinement,''
  Eur.\ Phys.\ J.\ C {\bf 22}, 463 (2001)
  %doi:10.1007/s100520100821
  [hep-th/0010079].
  %%CITATION = doi:10.1007/s100520100821;%%
  %18 citations counted in INSPIRE as of 15 Apr 2017
	
%\cite{Chaichian:2005vt}
\bibitem{Chaichian:2005vt} 
  M.~Chaichian and K.~Nishijima,
  %``Does colour confinement imply massive gluons?,''
  Eur.\ Phys.\ J.\ C {\bf 47}, 737 (2006)
  %doi:10.1140/epjc/s2006-02592-8
  [hep-th/0504050].
  %%CITATION = doi:10.1140/epjc/s2006-02592-8;%%
  %10 citations counted in INSPIRE as of 21 Apr 2017
	
%\cite{Nishijima:2007ry}
\bibitem{Nishijima:2007ry} 
  K.~Nishijima and A.~Tureanu,
  %``Gauge-dependence of Green's functions in QCD and QED,''
  Eur.\ Phys.\ J.\ C {\bf 53}, 649 (2008)
  %doi:10.1140/epjc/s10052-007-0486-1
  [arXiv:0710.1257 [hep-th]].
  %%CITATION = doi:10.1140/epjc/s10052-007-0486-1;%%
  %2 citations counted in INSPIRE as of 18 Apr 2017
	
%\cite{Seiberg:1994aj}
\bibitem{Seiberg:1994aj} 
  N.~Seiberg and E.~Witten,
  %``Monopoles, duality and chiral symmetry breaking in N=2 supersymmetric QCD,''
  Nucl.\ Phys.\ B {\bf 431}, 484 (1994)
  %doi:10.1016/0550-3213(94)90214-3
  [hep-th/9408099].
  %%CITATION = doi:10.1016/0550-3213(94)90214-3;%%
  %2098 citations counted in INSPIRE as of 02 May 2017
	
%\cite{Seiberg:1994rs}
\bibitem{Seiberg:1994rs} 
  N.~Seiberg and E.~Witten,
  %``Electric - magnetic duality, monopole condensation, and confinement in N=2 supersymmetric Yang--Mills theory,''
  Nucl.\ Phys.\ B {\bf 426}, 19 (1994)
  Erratum: [Nucl.\ Phys.\ B {\bf 430}, 485 (1994)]
  %doi:10.1016/0550-3213(94)90124-4, 10.1016/0550-3213(94)00449-8
  [hep-th/9407087].
  %%CITATION = doi:10.1016/0550-3213(94)90124-4, 10.1016/0550-3213(94)00449-8;%%
  %2882 citations counted in INSPIRE as of 02 May 2017
	
%\cite{Chaichian:1999is}
\bibitem{Chaichian:1999is} 
  M.~Chaichian and T.~Kobayashi,
  %``On different criteria for confinement,''
  Phys.\ Lett.\ B {\bf 481}, 26 (2000)
  %doi:10.1016/S0370-2693(00)00438-X
  [hep-th/9903103].
  %%CITATION = doi:10.1016/S0370-2693(00)00438-X;%%
  %1 citations counted in INSPIRE as of 18 Aug 2017
	
%\cite{Gribov:1977wm}
\bibitem{Gribov:1977wm} 
  V.~N.~Gribov,
  %``Quantization of Nonabelian Gauge Theories,''
  Nucl.\ Phys.\ B {\bf 139}, 1 (1978).
  %doi:10.1016/0550-3213(78)90175-X
  %%CITATION = doi:10.1016/0550-3213(78)90175-X;%%
  %1550 citations counted in INSPIRE as of 28 Jul 2017
	
%\cite{Zwanziger:1989mf}
\bibitem{Zwanziger:1989mf} 
  D.~Zwanziger,
  %``Local and Renormalizable Action From the Gribov Horizon,''
  Nucl.\ Phys.\ B {\bf 323}, 513 (1989).
  %doi:10.1016/0550-3213(89)90122-3
  %%CITATION = doi:10.1016/0550-3213(89)90122-3;%%
  %351 citations counted in INSPIRE as of 28 Jul 2017
	
%\cite{Bogolubsky:2007ud}
\bibitem{Bogolubsky:2007ud}
  I.~L.~Bogolubsky, E.~M.~Ilgenfritz, M.~Muller-Preussker, A.~Sternbeck,
  %``The Landau gauge gluon and ghost propagators in 4D SU(3) gluodynamics in large lattice volumes,''
  PoS LAT2007, 290 (2007).
  %[arXiv:0710.1968 [hep-lat]].
  
%\cite{Cucchieri:2007md}
\bibitem{Cucchieri:2007md}
  A.~Cucchieri, T.~Mendes,
  %``What's up with IR gluon and ghost propagators in Landau gauge? A puzzling answer from huge lattices,''
  PoS LAT2007, 297 (2007).
  %[arXiv:0710.0412 [hep-lat]]. 
   
%\cite{Oliveira:2007px}
\bibitem{Oliveira:2007px}
  O.~Oliveira, P.~J.~Silva, E.~M.~Ilgenfritz, A.~Sternbeck,
  %``The Gluon propagator from large asymmetric lattices,''
  PoS LAT2007, 323 (2007).
  %[arXiv:0710.1424 [hep-lat]].
	
%\cite{Lucini:2004my}
\bibitem{Lucini:2004my} 
  B.~Lucini, M.~Teper and U.~Wenger,
  %``Glueballs and k-strings in SU(N) gauge theories: Calculations with improved operators,''
  JHEP {\bf 0406}, 012 (2004).
  %doi:10.1088/1126-6708/2004/06/012
  %[hep-lat/0404008].
  %%CITATION = doi:10.1088/1126-6708/2004/06/012;%%
  %145 citations counted in INSPIRE as of 14 févr. 2016
	
%\cite{Chen:2005mg}
\bibitem{Chen:2005mg} 
  Y.~Chen {\it et al.},
  %``Glueball spectrum and matrix elements on anisotropic lattices,''
  Phys.\ Rev.\ D {\bf 73}, 014516 (2006).
  %doi:10.1103/PhysRevD.73.014516
  %[hep-lat/0510074].
  %%CITATION = doi:10.1103/PhysRevD.73.014516;%%
  %311 citations counted in INSPIRE as of 14 févr. 2016

%%%%% Theoretical understanding of Yang--Mills thoery %%%%%%%%%%

%\cite{Cornwall:1981zr}
\bibitem{Cornwall:1981zr} 
  J.~M.~Cornwall,
  %``Dynamical Mass Generation in Continuum QCD,''
  Phys.\ Rev.\ D {\bf 26}, 1453 (1982).
  %%CITATION = PHRVA,D26,1453;%%
  %806 citations counted in INSPIRE as of 04 Jun 2015
	
\bibitem{Cornwall:2010bk}	
	J.~M.~Cornwall, J.~Papavassiliou, D.~Binosi, 
  ``The Pinch Technique and its Applications to Non-Abelian Gauge Theories'', 	
	(Cambridge University Press, Cambridge, 2010).	

%\cite{Dudal:2008sp}
\bibitem{Dudal:2008sp} 
  D.~Dudal, J.~A.~Gracey, S.~P.~Sorella, N.~Vandersickel and H.~Verschelde,
  %``A Refinement of the Gribov-Zwanziger approach in the Landau gauge: Infrared propagators in harmony with the lattice results,''
  Phys.\ Rev.\ D {\bf 78}, 065047 (2008)
  [arXiv:0806.4348 [hep-th]].
  %%CITATION = ARXIV:0806.4348;%%
  %283 citations counted in INSPIRE as of 04 Jun 2015
	  
%\cite{Frasca:2007uz}
\bibitem{Frasca:2007uz} 
  M.~Frasca,
  %``Infrared Gluon and Ghost Propagators,''
  Phys.\ Lett.\ B {\bf 670}, 73 (2008)
  [arXiv:0709.2042 [hep-th]].
  %%CITATION = ARXIV:0709.2042;%%
	  
%\cite{Frasca:2009yp}
\bibitem{Frasca:2009yp}
  M.~Frasca,
  %``Mapping a Massless Scalar Field Theory on a Yang--Mills Theory: Classical Case,''
  Mod.\ Phys.\ Lett.\  {\bf A24}, 2425-2432 (2009)
  [arXiv:0903.2357 [math-ph]].
	
%\cite{Frasca:2015yva}
\bibitem{Frasca:2015yva} 
  M.~Frasca,
  %``Quantum Yang--Mills field theory,''
  Eur.\ Phys.\ J.\ Plus {\bf 132}, no. 1, 38 (2017)
  Erratum: [Eur.\ Phys.\ J.\ Plus {\bf 132}, no. 5, 242 (2017)]
  %doi:10.1140/epjp/i2017-11563-0, 10.1140/epjp/i2017-11321-4
  [arXiv:1509.05292 [math-ph]].
  %%CITATION = doi:10.1140/epjp/i2017-11563-0, 10.1140/epjp/i2017-11321-4;%%
  %8 citations counted in INSPIRE as of 21 Nov 2017
	
%%%% Nesterenko %%%%%%

%%\cite{Nesterenko:1999np}
%\bibitem{Nesterenko:1999np} 
%  A.~V.~Nesterenko,
%  %``Quark - anti-quark potential in the analytic approach to QCD,''
% Phys.\ Rev.\ D {\bf 62}, 094028 (2000),
%  %doi:10.1103/PhysRevD.62.094028
%  [hep-ph/9912351].
%  %%CITATION = doi:10.1103/PhysRevD.62.094028;%%
%  %76 citations counted in INSPIRE as of 17 Aug 2016

%%\cite{Nesterenko:2001st}
%\bibitem{Nesterenko:2001st} 
%  A.~V.~Nesterenko,
%  %``New analytic running coupling in space - like and time - like regions,''
%  Phys.\ Rev.\ D {\bf 64}, 116009 (2001),
%  %doi:10.1103/PhysRevD.64.116009
%  [hep-ph/0102124].
%  %%CITATION = doi:10.1103/PhysRevD.64.116009;%%
% %63 citations counted in INSPIRE as of 17 Aug 2016
	
%%\cite{Nesterenko:2003xb}
%\bibitem{Nesterenko:2003xb} 
%  A.~V.~Nesterenko,
%  %``Analytic invariant charge in QCD,''
%  Int.\ J.\ Mod.\ Phys.\ A {\bf 18}, 5475 (2003),
%  %doi:10.1142/S0217751X0301704X
%  [hep-ph/0308288].
%  %%CITATION = doi:10.1142/S0217751X0301704X;%%
%  %79 citations counted in INSPIRE as of 17 Aug 2016

%%\cite{Baldicchi:2007ic}
%\bibitem{Baldicchi:2007ic} 
  %M.~Baldicchi, A.~V.~Nesterenko, G.~M.~Prosperi, D.~V.~Shirkov and C.~Simolo,
  %%``Bound state approach to the QCD coupling at low energy scales,''
  %Phys.\ Rev.\ Lett.\  {\bf 99}, 242001 (2007),
  %%doi:10.1103/PhysRevLett.99.242001
  %[arXiv:0705.0329 [hep-ph]].
  %%%CITATION = doi:10.1103/PhysRevLett.99.242001;%%
  %%47 citations counted in INSPIRE as of 17 Aug 2016
%
%%\cite{Baldicchi:2007zn}
%\bibitem{Baldicchi:2007zn} 
  %M.~Baldicchi, A.~V.~Nesterenko, G.~M.~Prosperi and C.~Simolo,
  %%``QCD coupling below 1 GeV from quarkonium spectrum,''
  %Phys.\ Rev.\ D {\bf 77}, 034013 (2008),
  %%doi:10.1103/PhysRevD.77.034013
  %[arXiv:0705.1695 [hep-ph]].
  %%%CITATION = doi:10.1103/PhysRevD.77.034013;%%
  %%39 citations counted in INSPIRE as of 17 Aug 2016
	%
%%%%% Running coupling on lattice %%%%%%
	%
%%\cite{Bogolubsky:2009dc}
%\bibitem{Bogolubsky:2009dc}
  %I.~L.~Bogolubsky, E.~M.~Ilgenfritz, M.~Muller-Preussker, A.~Sternbeck,
  %%``Lattice gluodynamics computation of Landau gauge Green's functions in the deep infrared,''
  %Phys.\ Lett.\  {\bf B676}, 69-73 (2009),
  %[arXiv:0901.0736 [hep-lat]].
	%
%%\cite{Duarte:2016iko}
%\bibitem{Duarte:2016iko} 
  %A.~G.~Duarte, O.~Oliveira and P.~J.~Silva,
  %%``Lattice Gluon and Ghost Propagators, and the Strong Coupling in Pure SU(3) Yang--Mills Theory: Finite Lattice Spacing and Volume Effects,''
  %Phys.\ Rev.\ D {\bf 94}, no. 1, 014502 (2016),
  %%doi:10.1103/PhysRevD.94.014502
  %[arXiv:1605.00594 [hep-lat]].
  %%%CITATION = doi:10.1103/PhysRevD.94.014502;%%
  %%5 citations counted in INSPIRE as of 17 Aug 2016
	%
%\cite{Deur:2016tte}
\bibitem{Deur:2016tte} 
  A.~Deur, S.~J.~Brodsky and G.~F.~de Teramond,
  %``The QCD Running Coupling,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 90}, 1 (2016),
  %doi:10.1016/j.ppnp.2016.04.003
  [arXiv:1604.08082 [hep-ph]].
  %%CITATION = doi:10.1016/j.ppnp.2016.04.003;%%
  %9 citations counted in INSPIRE as of 24 Aug 2016
	
%\cite{Deur:2016bwq}
\bibitem{Deur:2016bwq} 
  A.~Deur,
  %``Self-interacting scalar fields at high-temperature,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 6, 412 (2017)
  %doi:10.1140/epjc/s10052-017-4971-x
  [arXiv:1611.05515 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-4971-x;%%
  %2 citations counted in INSPIRE as of 18 Oct 2017

  %
 %\bibitem{Olive:2016xmw} 
  %C.~Patrignani {\it et al.} [Particle Data Group],
  %%``Review of Particle Physics,''
  %Chin.\ Phys.\ C {\bf 40}, no. 10, 100001 (2016).
 %% doi:10.1088/1674-1137/40/10/100001
  %%%CITATION = doi:10.1088/1674-1137/40/10/100001;%%
  %%1147 citations counted in INSPIRE as of 10 Jul 2017
	
	

% %\cite{Frasca:2015yva}
% \bibitem{Frasca:2015yva} 
% M.~Frasca,
% %``Quantum Yang-Mills field theory,''
% Eur.\ Phys.\ J.\ Plus {\bf 132}, no. 1, 38 (2017)
% Erratum: [Eur.\ Phys.\ J.\ Plus {\bf 132}, no. 5, 242 (2017)]
% doi:10.1140/epjp/i2017-11563-0, 10.1140/epjp/i2017-11321-4
% [arXiv:1509.05292 [math-ph]].
% %%CITATION = doi:10.1140/epjp/i2017-11563-0, 10.1140/epjp/i2017-11321-4;%%
% %8 citations counted in INSPIRE as of 21 Nov 2017



  
%%\cite{Buoninfante:2018mre}
%\bibitem{Buoninfante:2018mre}
%L.~Buoninfante, G.~Lambiase and A.~Mazumdar,
%%``Ghost-free infinite derivative quantum field theory,''
%Nucl. Phys. B \textbf{944}, 114646 (2019)
%doi:10.1016/j.nuclphysb.2019.114646
%[arXiv:1805.03559 [hep-th]].
%%49 citations counted in INSPIRE as of 18 Nov 2020



%\cite{Kimura:2016irk}
\bibitem{Kimura:2016irk}
T.~Kimura, A.~Mazumdar, T.~Noumi and M.~Yamaguchi,
%``Nonlocal $ \mathcal{N}=1 $ supersymmetry,''
JHEP \textbf{10}, 022 (2016)
doi:10.1007/JHEP10(2016)022
[arXiv:1608.01652 [hep-th]].
%16 citations counted in INSPIRE as of 24 Jan 2021

%\cite{Pius:2016jsl}
\bibitem{Pius:2016jsl}
R.~Pius and A.~Sen,
%``Cutkosky rules for superstring field theory,''
JHEP \textbf{10}, 024 (2016)
[erratum: JHEP \textbf{09}, 122 (2018)]
doi:10.1007/JHEP10(2016)024
[arXiv:1604.01783 [hep-th]].
%63 citations counted in INSPIRE as of 17 Apr 2021

%\cite{Briscese:2018oyx}
\bibitem{Briscese:2018oyx}
F.~Briscese and L.~Modesto,
%``Cutkosky rules and perturbative unitarity in Euclidean nonlocal quantum field theories,''
Phys. Rev. D \textbf{99}, no.10, 104043 (2019)
doi:10.1103/PhysRevD.99.104043
[arXiv:1803.08827 [gr-qc]].
%31 citations counted in INSPIRE as of 17 Apr 2021


%\cite{Briscese:2018oyx}
\bibitem{Briscese:2018oyx}
F.~Briscese and L.~Modesto,
%``Cutkosky rules and perturbative unitarity in Euclidean nonlocal quantum field theories,''
Phys. Rev. D \textbf{99}, no.10, 104043 (2019)
doi:10.1103/PhysRevD.99.104043
[arXiv:1803.08827 [gr-qc]].
%47 citations counted in INSPIRE as of 01 Mar 2022

%\cite{Koshelev:2020fok}
\bibitem{Koshelev:2020fok}
A.~S.~Koshelev and A.~Tokareva,
%``Non-local self-healing of Higgs inflation,''
Phys. Rev. D \textbf{102}, 123518 (2020)
doi:10.1103/PhysRevD.102.123518
[arXiv:2006.06641 [hep-th]].
%4 citations counted in INSPIRE as of 17 Apr 2021





%\cite{Briscese:2021mob}
\bibitem{Briscese:2021mob}
F.~Briscese and L.~Modesto,
%``Non-unitarity of Minkowskian non-local quantum field theories,''
Eur. Phys. J. C \textbf{81}, no.8, 730 (2021)
doi:10.1140/epjc/s10052-021-09525-7
[arXiv:2103.00353 [hep-th]].
%12 citations counted in INSPIRE as of 01 Mar 2022

%\cite{Koshelev:2021orf}
\bibitem{Koshelev:2021orf}
A.~S.~Koshelev and A.~Tokareva,
%``Unitarity of Minkowski non-local theories made explicit,''
[arXiv:2103.01945 [hep-th]].
%1 citations counted in INSPIRE as of 17 Apr 2021




\bibitem{Sundrum} C.~Kilic, T.~Okui and R.~Sundrum,
  %``Vectorlike Confinement at the LHC,''
  JHEP {1002}, 018 (2010)
  [\hhref{0906.0577}].

\bibitem{FN}
 M.~Farina, D.~Pappadopulo and A.~Strumia,
  %``A modified naturalness principle and its experimental tests,''
  JHEP {1308}, 022 (2013)
  [\hhref{1303.7244}].
   A.~de Gouvea, D.~Hernandez and T.~M.~P.~Tait,
  %``Criteria for Natural Hierarchies,''
  Phys.\ Rev.\ D {89} (2014) 115005
  [\hhref{1402.2658}].

\bibitem{Bardeen}
F. Englert, C. Truffin and R. Gastmans, Nucl. Phys. B 117 (1976) 407.
W Bardeen, \href{http://lss.fnal.gov/archive/1995/conf/Conf-95-391-T.pdf}{FERMILAB-CONF-95-391-T}.
C.~T.~Hill,
  %``Conjecture on the physical implications of the scale anomaly,''
  \hhref{hep-th/0510177}.
 
\bibitem{agrav}
  A.~Salvio and A.~Strumia,
  %``Agravity,''
  JHEP {1406} (2014) 080
  [\hhref{1403.4226}].
  
  \bibitem{prev}   
R. Hempfling,
 %``The Next-to-minimal Coleman-Weinberg model,''
  Phys.\ Lett.\ B {379} (1996) 153
  [\hhref{hep-ph/9604278}].
   J.~P.~Fatelo, J.~M.~Gerard, T.~Hambye and J.~Weyers,
  %``Symmetry breaking induced by top loops,''
  Phys.\ Rev.\ Lett.\  {74} (1995) 492.
  T.~Hambye,
  %``Symmetry breaking induced by top quark loops from a model without scalar mass,''
  Phys.\ Lett.\ B {371} (1996) 87
  [\hhref{hep-ph/9510266}].
  W.~-F.~Chang, J.~N.~Ng and J.~M.~S.~Wu,
  %``Shadow Higgs from a scale-invariant hidden U(1)(s) model,''
  Phys.\ Rev.\ D {75} (2007) 115016
  [\hhref{hep-ph/0701254}].
  R.~Foot, A.~Kobakhidze and R.~R.~Volkas,
  %``electro-weak Higgs as a pseudo-Goldstone boson of broken scale invariance,''
  Phys.\ Lett.\ B {655} (2007) 156
  [\hhref{0704.1165}].
R.~Foot, A.~Kobakhidze, K.~L.~McDonald, R.~R.~Volkas,
  %``A Solution to the hierarchy problem from an almost decoupled hidden sector within a classically scale invariant theory,''
  Phys.\ Rev.\ D {77} (2008) 035006
  [\hhref{0709.2750}].
    S.~Iso, N.~Okada, Y.~Orikasa,
  %``The minimal B-L model naturally realized at TeV scale,''
  Phys.\ Rev.\ D {80} (2009) 115007
  [\hhref{0909.0128}].
  S.~Iso and Y.~Orikasa,
  %``TeV Scale B-L model with a flat Higgs potential at the Planck scale - in view of the hierarchy problem -,''
  PTEP {2013} (2013) 023B08
  [\hhref{1210.2848}].
C.~Englert, J.~Jaeckel, V.~V.~Khoze and M.~Spannowsky,
 %``Emergence of the electro-weak Scale through the Higgs Portal,''
  \hhref{1301.4224}.
   E.J.~Chun, S. Jung, H.M.~Lee,
  %``Vacuum Stability, Perturbativity, EWPD and Higgs-to-diphoton in Type II Seesaw,''
  \hhref{1304.5815}.
  T.~Hambye and A.~Strumia,
  %``Dynamical generation of the weak and Dark Matter scale,''
  Phys.\ Rev.\ D {88} (2013) 055022
  [\hhref{1306.2329}].
  C.~D.~Carone and R.~Ramos,
  %``Classical scale-invariance, the electro-weak scale and vector dark matter,''
  Phys.\ Rev.\ D {88} (2013) 055020
  [\hhref{1307.8428}].
   R.~Foot, A.~Kobakhidze, K.~L.~McDonald and R.~R.~Volkas,
  %``Poincare Protection for a Natural electro-weak Scale,''
  Phys.\ Rev.\ D {89} (2014) 115018
  [\hhref{1310.0223}].
    A.~Farzinnia, H.~J.~He and J.~Ren,
  %``Natural Electroweak Symmetry Breaking from Scale Invariant Higgs Mechanism,''
  Phys.\ Lett.\ B {727} (2013) 141
  [arXiv:1308.0295].
  C.~T.~Hill,
  %``Is the Higgs Boson Associated with Coleman-Weinberg Dynamical Symmetry Breaking?,''
  Phys.\ Rev.\ D {89} (2014) 073003
  [\hhref{1401.4185}.
  J.~Guo and Z.~Kang,
  %``Higgs Naturalness and Dark Matter Stability by Scale Invariance,''
  \hhref{1401.5609}.
  S.~Benic and B.~Radovcic,
  %``electro-weak breaking and Dark Matter from the common scale,''
  Phys.\ Lett.\ B {732} (2014) 91
  [\hhref{1401.8183}].
   H.~Davoudiasl, I.M.~Lewis, 
  %``Right-Handed Neutrinos as the Origin of the Electroweak Scale,''
  Phys.\ Rev.\ D {90}, 033003 (2014)   [\hhref{1404.6260}].
K.~Allison, C.~T.~Hill and G.~G.~Ross,   \hhref{1404.6268}.
  %``Ultra-weak sector, Higgs boson mass, and the dilaton,''
   G.~M.~Pelaggi,
  %``Predictions of a model of weak scale from dynamical breaking of scale invariance,''
  \hhref{1406.4104}. 
  W.~Altmannshofer, W.~A.~Bardeen, M.~Bauer, M.~Carena and J.~D.~Lykken,
  %``Light Dark Matter, Naturalness, and the Radiative Origin of the electro-weak Scale,''
  \hhref{1408.3429}.
  
 
\bibitem{Raidal}
T.~Hur and P.~Ko,
  %``Scale invariant extension of the standard model with strongly interacting hidden sector,''
  Phys.\ Rev.\ Lett.\  {106}, 141802 (2011)
  [\hhref{1103.2571}].  
  M.~Heikinheimo, A.~Racioppi, M.~Raidal, C.~Spethmann and K.~Tuominen,
  %``Physical Naturalness and Dynamical Breaking of Classical Scale Invariance,''
  Mod.\ Phys.\ Lett.\ A {29} (2014) 1450077
  [\hhref{1304.7006}].
  


  
%%\cite{Ghoshal:2020lfd}
%\bibitem{Ghoshal:2020lfd}
%A.~Ghoshal, A.~Mazumdar, N.~Okada and D.~Villalba,
%``Non-local Non-Abelian Gauge Theory: Conformal Invariance %and $\beta$-function,''
%[arXiv:2010.15919 [hep-ph]].
%%0 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Chaichian:2018cyv}
\bibitem{Chaichian:2018cyv}
M.~Chaichian and M.~Frasca,
%``Condition for confinement in non-Abelian gauge theories,''
Phys. Lett. B \textbf{781}, 33-39 (2018)
doi:10.1016/j.physletb.2018.03.067
[arXiv:1801.09873 [hep-th]].
9 citations counted in INSPIRE as of 16 Jan 2021


%\bibitem{Tomboulis:1997gg} 
%E.~T.~Tomboulis, 
%%%"Superrenormalizable gauge and gravitational theories,"
%hep-th/9702146.




%\cite{Peskin:1995ev}
\bibitem{Peskin:1995ev}
M.~E.~Peskin and D.~V.~Schroeder,
``An Introduction to quantum field theory,''
(Perseus Books Publishing, Reading, 1995).
%1422 citations counted in INSPIRE as of 21 Dec 2020


%\cite{Bender:1999ek}
\bibitem{Bender:1999ek} 
C.~M.~Bender, K.~A.~Milton and V.~M.~Savage,
%``Solution of Schwinger-Dyson equations for PT symmetric quantum field theory,''
Phys.\ Rev.\ D {\bf 62}, 085001 (2000)
[hep-th/9907045].
%%CITATION = HEP-TH/9907045;%%
%50 citations counted in INSPIRE as of 04 sept. 2015
 



%\cite{Klevansky:1992qe}
\bibitem{Klevansky:1992qe}
S.~P.~Klevansky,
%``The Nambu-Jona-Lasinio model of quantum chromodynamics,''
Rev. Mod. Phys. \textbf{64}, 649-708 (1992)
doi:10.1103/RevModPhys.64.649
%1656 citations counted in INSPIRE as of 24 Jan 2021


  
%\cite{Chun:2019box}
\bibitem{Chun:2019box}
E.~J.~Chun and C.~Han,
%``A scalar potential from gauge condensation and its implications,''
Eur. Phys. J. C \textbf{80}, no.10, 977 (2020)
doi:10.1140/epjc/s10052-020-08543-1
[arXiv:1911.01050 [hep-ph]].
%0 citations counted in INSPIRE as of 08 Feb 2021

%\cite{Narison:2011xe}
\bibitem{Narison:2011xe}
S.~Narison,
%``Gluon Condensates and precise $\overline{m}_{c,b}$ from QCD-Moments and their ratios to Order $\alpha_s^3$ and \ensuremath{<} G$^4$ \ensuremath{>},''
Phys. Lett. B \textbf{706}, 412-422 (2012)
doi:10.1016/j.physletb.2011.11.058
[arXiv:1105.2922 [hep-ph]].
%109 citations counted in INSPIRE as of 30 Mar 2021

\bibitem{Lindner}  
T.~Hambye and M.~H.~G.~Tytgat,
  %``Confined hidden vector dark matter,''
  Phys.\ Lett.\ B {683} (2010) 39
  [\hhref{0907.1007}].  
  M.~Holthausen, J.~Kubo, K.~S.~Lim and M.~Lindner,
  %``electro-weak and Conformal Symmetry Breaking by a Strongly Coupled Hidden Sector,''
  JHEP {1312} (2013) 076
  [\hhref{1310.4423}].
  %See also~\cite{LindnerQCD}.






%%\cite{Frasca:2009yp}
%\bibitem{Frasca:2009yp}
%M.~Frasca,
%%``Mapping a Massless Scalar Field Theory on a Yang-Mills Theory: Classical Case,''
%Mod. Phys. Lett. A \textbf{24}, 2425-2432 (2009)
%doi:10.1142/S021773230903165X
%[arXiv:0903.2357 [math-ph]].
%%37 citations counted in INSPIRE as of 28 Sep 2020
%
%%\cite{Frasca:2007uz}
%\bibitem{Frasca:2007uz}
%M.~Frasca,
%%``Infrared Gluon and Ghost Propagators,''
%Phys. Lett. B \textbf{670}, 73-77 (2008)
%doi:10.1016/j.physletb.2008.10.022
%[arXiv:0709.2042 [hep-th]].
%%66 citations counted in INSPIRE as of 28 Sep 2020
%
%%\cite{Frasca:2013tma}
%\bibitem{Frasca:2013tma}
%M.~Frasca,
%%``Scalar field theory in the strong self-interaction limit,''
%Eur. Phys. J. C \textbf{74}, 2929 (2014)
%doi:10.1140/epjc/s10052-014-2929-9
%[arXiv:1306.6530 [hep-ph]].
%%16 citations counted in INSPIRE as of 15 Nov 2020
	%
%%\cite{Frasca:2017slg}
%\bibitem{Frasca:2017slg} 
%M.~Frasca,
%%``Spectrum of Yang-Mills theory in 3 and 4 dimensions,''
%Nucl.\ Part.\ Phys.\ Proc.\  {\bf 294-296}, 124 (2018)
%doi:10.1016/j.nuclphysbps.2018.02.005
%[arXiv:1708.06184 [hep-ph]].
%%%CITATION = doi:10.1016/j.nuclphysbps.2018.02.005;%%
%%1 citations counted in INSPIRE as of 28 Nov 2018
%
%%\cite{Frasca:2019ysi}
%\bibitem{Frasca:2019ysi}
%M.~Frasca,
%%``Differential DysonSchwinger equations for quantum chromodynamics,''
%Eur. Phys. J. C \textbf{80}, no.8, 707 (2020)
%doi:10.1140/epjc/s10052-020-8261-7
%[arXiv:1901.08124 [hep-ph]].
%%0 citations counted in INSPIRE as of 06 Sep 2020
%
%%\cite{Smilga:2001ck}
%\bibitem{Smilga:2001ck}
%A.~V.~Smilga,
%``Lectures on quantum chromodynamics,'', (World Scientific, Singapore, 2001).
%%25 citations counted in INSPIRE as of 10 Oct 2020
%
%
%%\cite{Wu:1967vp}
%\bibitem{Wu:1967vp}
%T.~T.~Wu and C.~N.~Yang,
%``SOME SOLUTIONS OF THE CLASSICAL ISOTOPIC GAUGE FIELD EQUATIONS,''
%Published in: In Yang, C.N.: Selected Papers 1945-1980*, 400-405 also in H. Mark and S. Fernbach, Properties Of Matter Under Unusual Conditions*, New York 1969, 349-345,
%PRINT-67-2362.
%%1 citations counted in INSPIRE as of 29 Dec 2020
%
%%\cite{Kugo:1977zq}
%\bibitem{Kugo:1977zq}
%T.~Kugo and I.~Ojima,
%%``Manifestly Covariant Canonical Formulation of Yang-Mills Field Theories: Physical State Subsidiary Conditions and Physical S Matrix Unitarity,''
%Phys. Lett. B \textbf{73}, 459-462 (1978)
%doi:10.1016/0370-2693(78)90765-7
%%303 citations counted in INSPIRE as of 29 Dec 2020
%
%%\cite{Kugo:1979gm}
%\bibitem{Kugo:1979gm}
%T.~Kugo and I.~Ojima,
%%``Local Covariant Operator Formalism of Nonabelian Gauge Theories and Quark Confinement Problem,''
%Prog. Theor. Phys. Suppl. \textbf{66}, 1-130 (1979)
%doi:10.1143/PTPS.66.1
%%1036 citations counted in INSPIRE as of 29 Dec 2020
	%
%%%\cite{Chaichian:2018cyv}
%%\bibitem{Chaichian:2018cyv} 
%%M.~Chaichian and M.~Frasca,
%%%``Condition for confinement in non-Abelian gauge theories,''
%%Phys.\ Lett.\ B {\bf 781}, 33 (2018)
%%doi:10.1016/j.physletb.2018.03.067
%%[arXiv:1801.09873 [hep-th]].
%%%%CITATION = doi:10.1016/j.physletb.2018.03.067;%%
%%%1 citations counted in INSPIRE as of 31 Aug 2018
%
%%\cite{Boddy:2014yra}
%\bibitem{Boddy:2014yra}
%K.~K.~Boddy, J.~L.~Feng, M.~Kaplinghat and T.~M.~P.~Tait,
%%``Self-Interacting Dark Matter from a Non-Abelian Hidden Sector,''
%Phys. Rev. D \textbf{89}, no.11, 115017 (2014)
%doi:10.1103/PhysRevD.89.115017
%[arXiv:1402.3629 [hep-ph]].
%%158 citations counted in INSPIRE as of 04 Jan 2021
%
%%\cite{Boddy:2014qxa}
%\bibitem{Boddy:2014qxa}
%K.~K.~Boddy, J.~L.~Feng, M.~Kaplinghat, Y.~Shadmi and T.~M.~P.~Tait,
%%``Strongly interacting dark matter: Self-interactions and keV lines,''
%Phys. Rev. D \textbf{90}, no.9, 095016 (2014)
%doi:10.1103/PhysRevD.90.095016
%[arXiv:1408.6532 [hep-ph]].
%%70 citations counted in INSPIRE as of 04 Jan 2021
%
%%\cite{Modesto:2011kw}
%\bibitem{Modesto:2011kw}
%L.~Modesto,
%%``Super-renormalizable Quantum Gravity,''
%Phys. Rev. D \textbf{86}, 044005 (2012)
%doi:10.1103/PhysRevD.86.044005
%[arXiv:1107.2403 [hep-th]].
%%352 citations counted in INSPIRE as of 04 Jan 2021
%
%
%
%%\begin{thebibliography}{99}
%
%%% \bibitem{label}
%%% Text of bibliographic item
%
%%%\cite{Greensite:2011zz}
%%\bibitem{Greensite:2011zz} 
%%  J.~Greensite,
%%  ``An introduction to the confinement problem,''
%%  Lect.\ Notes Phys.\ {\bf 821}, (Springer, Berlin, 2011).
%%  %doi:10.1007/978-3-642-14382-3
%%  %%CITATION = doi:10.1007/978-3-642-14382-3;%%
%%  %82 citations counted in INSPIRE as of 18 Apr 2017
	%
%
	%
%%%%% Instanton liquid %%%%
    %
%%\cite{Schafer:1996wv}
%\bibitem{Schafer:1996wv}
  %T.~Sch\"afer and E.~V.~Shuryak,
  %%``Instantons in QCD,''
  %Rev.\ Mod.\ Phys.\  {\bf 70}, 323 (1998)
  %%[arXiv:hep-ph/9610451].
  %%%CITATION = RMPHA,70,323;%%
	%
%%\cite{Boucaud:2002fx}
%\bibitem{Boucaud:2002fx} 
  %P.~Boucaud, F.~De Soto, A.~Le Yaouanc, J.~P.~Leroy, J.~Micheli, H.~Moutarde, O.~Pene and J.~Rodriguez-Quintero,
  %%``The Strong coupling constant at small momentum as an instanton detector,''
  %JHEP {\bf 0304}, 005 (2003),
  %%doi:10.1088/1126-6708/2003/04/005
  %[hep-ph/0212192].
  %%%CITATION = doi:10.1088/1126-6708/2003/04/005;%%
  %%46 citations counted in INSPIRE as of 17 Aug 2016
	%
%%\cite{Frasca:2016sky}
%\bibitem{Frasca:2016sky} 
  %M.~Frasca,
  %%``Confinement in a three-dimensional Yang--Mills theory,''
  %Eur.\ Phys.\ J.\ C {\bf 77}, no. 4, 255 (2017)
  %%doi:10.1140/epjc/s10052-017-4824-7
  %[arXiv:1611.08182 [hep-th]].
  %%%CITATION = doi:10.1140/epjc/s10052-017-4824-7;%%
	%
%%\bibitem{KugoArg}	
%%	This argument is due to T.~Kugo, private communication.
	%
%%\cite{Bender:1999ek}
%\bibitem{Bender:1999ek} 
  %C.~M.~Bender, K.~A.~Milton and V.~M.~Savage,
  %%``Solution of Schwinger--Dyson equations for PT symmetric quantum field theory,''  
	%Phys.\ Rev.\ D {\bf 62}, 085001 (2000)  [hep-th/9907045].  
	%%%CITATION = HEP-TH/9907045;%%  
	%%50 citations counted in INSPIRE as of 17 sept. 2015
	%
%%%%% n-point functions on the lattice %%%%
%
%%\cite{Cucchieri:2008qm}
%\bibitem{Cucchieri:2008qm} 
  %A.~Cucchieri, A.~Maas and T.~Mendes,
  %%``Three-point vertices in Landau-gauge Yang--Mills theory,''
  %Phys.\ Rev.\ D {\bf 77}, 094510 (2008)
  %%doi:10.1103/PhysRevD.77.094510
  %[arXiv:0803.1798 [hep-lat]].
  %%%CITATION = doi:10.1103/PhysRevD.77.094510;%%
  %%106 citations counted in INSPIRE as of 18 Oct 2017
	%
%%\cite{Duarte:2016ieu}
%\bibitem{Duarte:2016ieu} 
  %A.~G.~Duarte, O.~Oliveira and P.~J.~Silva,
  %%``Further Evidence For Zero Crossing On The Three Gluon Vertex,''
  %Phys.\ Rev.\ D {\bf 94}, no. 7, 074502 (2016)
  %%doi:10.1103/PhysRevD.94.074502
  %[arXiv:1607.03831 [hep-lat]].
  %%%CITATION = doi:10.1103/PhysRevD.94.074502;%%
  %%11 citations counted in INSPIRE as of 18 Oct 2017	
	%
%%\cite{Sternbeck:2006rd}
%\bibitem{Sternbeck:2006rd} 
  %A.~Sternbeck,
  %%``The Infrared behavior of lattice QCD Green's functions,''
	%Ph.D. thesis (Advisor: Prof. M. M\"uller-Preu\ss ker), Humboldt-University Berlin, July 2006,
  %hep-lat/0609016.
  %%%CITATION = HEP-LAT/0609016;%%
  %%57 citations counted in INSPIRE as of 21 Nov 2017
	%
%%\cite{Aguilar:2009pp}
%\bibitem{Aguilar:2009pp} 
  %A.~C.~Aguilar, D.~Binosi and J.~Papavassiliou,
  %%``Indirect determination of the Kugo--Ojima function from lattice data,''
  %JHEP {\bf 0911}, 066 (2009)
  %%doi:10.1088/1126-6708/2009/11/066
  %[arXiv:0907.0153 [hep-ph]].
  %%%CITATION = doi:10.1088/1126-6708/2009/11/066;%%
  %%52 citations counted in INSPIRE as of 21 Nov 2017
	%
%\bibitem{PDG}
  %P.A. Zyla et al. (Particle Data Group), Prog. Theor. Exp. Phys. 2020, 083C01 (2020)
	%
%%\cite{Novikov:1983uc}
%\bibitem{Novikov:1983uc} 
  %V.~A.~Novikov, M.~A.~Shifman, A.~I.~Vainshtein and V.~I.~Zakharov,
  %%``Exact Gell-Mann-Low Function of Supersymmetric Yang--Mills Theories from Instanton Calculus,''
  %Nucl.\ Phys.\ B {\bf 229}, 381 (1983).
  %%doi:10.1016/0550-3213(83)90338-3
  %%%CITATION = doi:10.1016/0550-3213(83)90338-3;%%
  %%684 citations counted in INSPIRE as of 06 Jan 2018
	%
%%\cite{Shifman:1986zi}
%\bibitem{Shifman:1986zi} 
  %M.~A.~Shifman and A.~I.~Vainshtein,
  %%``Solution of the Anomaly Puzzle in SUSY Gauge Theories and the Wilson Operator Expansion,''
  %Nucl.\ Phys.\ B {\bf 277}, 456 (1986)
  %[Sov.\ Phys.\ JETP {\bf 64}, 428 (1986)]
  %[Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 91}, 723 (1986)].
  %%doi:10.1016/0550-3213(86)90451-7
  %%%CITATION = doi:10.1016/0550-3213(86)90451-7;%%
  %%519 citations counted in INSPIRE as of 06 Jan 2018
	%
%%\cite{Ryttov:2007cx}
%\bibitem{Ryttov:2007cx} 
  %T.~A.~Ryttov and F.~Sannino,
  %%``Supersymmetry inspired QCD beta function,''
  %Phys.\ Rev.\ D {\bf 78}, 065001 (2008)
  %%doi:10.1103/PhysRevD.78.065001
  %[arXiv:0711.3745 [hep-th]].
  %%%CITATION = doi:10.1103/PhysRevD.78.065001;%%
  %%154 citations counted in INSPIRE as of 06 Jan 2018
  
  
%\cite{Koshelev:2016vhi}
\bibitem{Koshelev:2016vhi}
A.~S.~Koshelev, K.~Sravan Kumar and P.~Vargas Moniz,
%``Effective models of inflation from a nonlocal framework,''
Phys. Rev. D \textbf{96}, no.10, 103503 (2017)
doi:10.1103/PhysRevD.96.103503
[arXiv:1604.01440 [hep-th]].
%22 citations counted in INSPIRE as of 20 Nov 2020

%\cite{SravanKumar:2018dlo}
\bibitem{SravanKumar:2018dlo}
K.~Sravan Kumar and L.~Modesto,
%``Non-local Starobinsky inflation in the light of future CMB,''
[arXiv:1810.02345 [hep-th]].
%8 citations counted in INSPIRE as of 20 Nov 2020

%\cite{Koshelev:2020fok}
\bibitem{Koshelev:2020fok}
A.~S.~Koshelev and A.~Tokareva,
%``Non-local self-healing of Higgs inflation,''
[arXiv:2006.06641 [hep-th]].
%1 citations counted in INSPIRE as of 20 Nov 2020

%\cite{Koshelev:2020xby}
\bibitem{Koshelev:2020xby}
A.~S.~Koshelev, K.~S.~Kumar and A.~A.~Starobinsky,
%``Analytic infinite derivative gravity, $R^2$-like inflation, quantum gravity and CMB,''
Int. J. Mod. Phys. D \textbf{29}, 2043018 (2020)
doi:10.1142/S021827182043018X
[arXiv:2005.09550 [hep-th]].
%5 citations counted in INSPIRE as of 20 Nov 2020

%\cite{Koshelev:2020foq}
\bibitem{Koshelev:2020foq}
A.~S.~Koshelev, K.~Sravan Kumar, A.~Mazumdar and A.~A.~Starobinsky,
%``Non-Gaussianities and tensor-to-scalar ratio in non-local R$^{2}$-like inflation,''
JHEP \textbf{06}, 152 (2020)
doi:10.1007/JHEP06(2020)152
[arXiv:2003.00629 [hep-th]].
%9 citations counted in INSPIRE as of 20 Nov 2020

%\cite{Krasnikov:2020kgh}
\bibitem{Krasnikov:2020kgh}
N.~V.~Krasnikov,
%``Nonlocal SU(5) GUT,''
Mod. Phys. Lett. A \textbf{36}, no.15, 2150104 (2021)
doi:10.1142/S0217732321501042
[arXiv:2012.10161 [hep-ph]].
%0 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2020ojd}
\bibitem{Frasca:2020ojd}
M.~Frasca and A.~Ghoshal,
%``Diluted mass gap in strongly coupled non-local Yang-Mills,''
JHEP \textbf{21}, 226 (2020)
doi:10.1007/JHEP07(2021)226
[arXiv:2102.10665 [hep-th]].
%6 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2020jbe}
\bibitem{Frasca:2020jbe}
M.~Frasca and A.~Ghoshal,
%``Mass gap in strongly coupled infinite derivative non-local Higgs: Dyson\textendash{}Schwinger approach,''
Class. Quant. Grav. \textbf{38}, no.17, 17 (2021)
doi:10.1088/1361-6382/ac161b
[arXiv:2011.10586 [hep-th]].
%7 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2021iip}
\bibitem{Frasca:2021iip}
M.~Frasca, A.~Ghoshal and N.~Okada,
%``Confinement and renormalization group equations in string-inspired nonlocal gauge theories,''
Phys. Rev. D \textbf{104}, no.9, 096010 (2021)
doi:10.1103/PhysRevD.104.096010
[arXiv:2106.07629 [hep-th]].
%3 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2022duz}
\bibitem{Frasca:2022duz}
M.~Frasca, A.~Ghoshal and A.~S.~Koshelev,
%``Non-perturbative Lee-Wick gauge theory: BRST, confinement \& RGE with strong couplings,''
[arXiv:2202.09578 [hep-ph]].
%1 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2022lwp}
\bibitem{Frasca:2022lwp}
M.~Frasca, A.~Ghoshal and S.~Groote,
%``Confinement in QCD and generic Yang-Mills theories with matter representations,''
[arXiv:2202.14023 [hep-ph]].
%0 citations counted in INSPIRE as of 03 Mar 2022

\bibitem{Biswas:2011ar} 
T.~Biswas, E.~Gerwick, T.~Koivisto and A.~Mazumdar,
%``Towards singularity and ghost free theories of gravity,''
Phys.\ Rev.\ Lett.\  {\bf 108}, 031101 (2012)
doi:10.1103/PhysRevLett.108.031101
[arXiv:1110.5249 [gr-qc]].
%%CITATION = doi:10.1103/PhysRevLett.108.031101;%%
%297 citations counted in INSPIRE as of 05 Mar 2018

%\cite{Giacchini:2018wlf}
\bibitem{Giacchini:2018wlf}
B.~L.~Giacchini and T.~de Paula Netto,
%``Effective delta sources and regularity in higher-derivative and ghost-free gravity,''
JCAP \textbf{07}, 013 (2019)
doi:10.1088/1475-7516/2019/07/013
[arXiv:1809.05907 [gr-qc]].
%26 citations counted in INSPIRE as of 06 Mar 2021

%\cite{Burzilla:2020utr}
\bibitem{Burzilla:2020utr}
N.~Burzill\`a, B.~L.~Giacchini, T.~d.~Netto and L.~Modesto,
%``Higher-order regularity in local and nonlocal quantum gravity,''
[arXiv:2012.11829 [gr-qc]].
%2 citations counted in INSPIRE as of 06 Mar 2021
  
  
\bibitem{Biswas:2013cha} 
T.~Biswas, A.~Conroy, A.~S.~Koshelev and A.~Mazumdar,
% ``Generalized ghost-free quadratic curvature gravity,''
Class.\ Quant.\ Grav.\  {\bf 31}, 015022 (2014)
Erratum: [Class.\ Quant.\ Grav.\  {\bf 31}, 159501 (2014)]
doi:10.1088/0264-9381/31/1/015022, 10.1088/0264-9381/31/15/159501
[arXiv:1308.2319 [hep-th]].
%%CITATION = doi:10.1088/0264-9381/31/1/015022, 10.1088/0264-9381/31/15/159501;%%
%86 citations counted in INSPIRE as of 10 Mar 2018
  
\bibitem{Frolov:2015bia} 
V.~P.~Frolov, A.~Zelnikov and T.~de Paula Netto,
% ``Spherical collapse of small masses in the ghost-free gravity,''
JHEP {\bf 1506}, 107 (2015)
doi:10.1007/JHEP06(2015)107
[arXiv:1504.00412 [hep-th]].
%%CITATION = doi:10.1007/JHEP06(2015)107;%%
%37 citations counted in INSPIRE as of 10 Mar 2018
  
  
\bibitem{Frolov:2015usa} 
V.~P.~Frolov and A.~Zelnikov
% ``Head-on collision of ultrarelativistic particles in ghost-free theories of gravity,''
Phys.\ Rev.\ D {\bf 93}, no. 6, 064048 (2016)
doi:10.1103/PhysRevD.93.064048
[arXiv:1509.03336 [hep-th]].
%%CITATION = doi:10.1103/PhysRevD.93.064048;%%
%26 citations counted in INSPIRE as of 10 Mar 2018
  
%\cite{Koshelev:2018hpt}
\bibitem{Koshelev:2018hpt}
A.~S.~Koshelev, J.~Marto and A.~Mazumdar,
%``Schwarzschild $1/r$-singularity is not permissible in ghost free quadratic curvature infinite derivative gravity,''
Phys. Rev. D \textbf{98}, no.6, 064023 (2018)
doi:10.1103/PhysRevD.98.064023
[arXiv:1803.00309 [gr-qc]].
%31 citations counted in INSPIRE as of 18 Nov 2020
  
\bibitem{Koshelev:2017bxd} 
A.~S.~Koshelev and A.~Mazumdar,
% ``Do massive compact objects without event horizon exist in infinite derivative gravity?,''
Phys.\ Rev.\ D {\bf 96}, no. 8, 084069 (2017)
doi:10.1103/PhysRevD.96.084069
[arXiv:1707.00273 [gr-qc]].
%%CITATION = doi:10.1103/PhysRevD.96.084069;%%
%12 citations counted in INSPIRE as of 10 Mar 2018
  
%\cite{Buoninfante:2018xiw}
\bibitem{Buoninfante:2018xiw}
L.~Buoninfante, A.~S.~Koshelev, G.~Lambiase and A.~Mazumdar,
%``Classical properties of non-local, ghost- and singularity-free gravity,''
JCAP \textbf{09}, 034 (2018)
doi:10.1088/1475-7516/2018/09/034
[arXiv:1802.00399 [gr-qc]].
%58 citations counted in INSPIRE as of 18 Nov 2020
  
\bibitem{Cornell:2017irh} 
A.~S.~Cornell, G.~Harmsen, G.~Lambiase and A.~Mazumdar,
%  ``Rotating metric in Non-Singular Infinite Derivative Theories of Gravity,''
arXiv:1710.02162 [gr-qc].
%%CITATION = ARXIV:1710.02162;%%
%5 citations counted in INSPIRE as of 10 Mar 2018
  
%\cite{Buoninfante:2018rlq}
\bibitem{Buoninfante:2018rlq}
L.~Buoninfante, A.~S.~Koshelev, G.~Lambiase, J.~Marto and A.~Mazumdar,
%``Conformally-flat, non-singular static metric in infinite derivative gravity,''
JCAP \textbf{06}, 014 (2018)
doi:10.1088/1475-7516/2018/06/014
[arXiv:1804.08195 [gr-qc]].
%41 citations counted in INSPIRE as of 18 Nov 2020

%\cite{Buoninfante:2018stt}
\bibitem{Buoninfante:2018stt}
L.~Buoninfante, G.~Harmsen, S.~Maheshwari and A.~Mazumdar,
%``Nonsingular metric for an electrically charged point-source in ghost-free infinite derivative gravity,''
Phys. Rev. D \textbf{98}, no.8, 084009 (2018)
doi:10.1103/PhysRevD.98.084009
[arXiv:1804.09624 [gr-qc]].
%31 citations counted in INSPIRE as of 18 Nov 2020

%\cite{Abel:2019zou}
\bibitem{Abel:2019zou}
S.~Abel, L.~Buoninfante and A.~Mazumdar,
%``Nonlocal gravity with worldline inversion symmetry,''
JHEP \textbf{01}, 003 (2020)
doi:10.1007/JHEP01(2020)003
[arXiv:1911.06697 [hep-th]].
%10 citations counted in INSPIRE as of 01 Dec 2020

%\cite{Buoninfante:2020ctr}
\bibitem{Buoninfante:2020ctr}
L.~Buoninfante, G.~Lambiase, Y.~Miyashita, W.~Takebe and M.~Yamaguchi,
%``Generalized ghost-free propagators in nonlocal field theories,''
Phys. Rev. D \textbf{101}, no.8, 084019 (2020)
doi:10.1103/PhysRevD.101.084019
[arXiv:2001.07830 [hep-th]].
%7 citations counted in INSPIRE as of 01 Dec 2020
  
\bibitem{Biswas:2005qr} 
T.~Biswas, A.~Mazumdar and W.~Siegel,
%``Bouncing universes in string-inspired gravity,''
JCAP {\bf 0603}, 009 (2006)
doi:10.1088/1475-7516/2006/03/009
[hep-th/0508194].
%%CITATION = doi:10.1088/1475-7516/2006/03/009;%%
%327 citations counted in INSPIRE as of 10 Mar 2018
  
\bibitem{Biswas:2006bs} 
T.~Biswas, R.~Brandenberger, A.~Mazumdar and W.~Siegel,
% ``Non-perturbative Gravity, Hagedorn Bounce and CMB,''
JCAP {\bf 0712}, 011 (2007)
doi:10.1088/1475-7516/2007/12/011
[hep-th/0610274].
%%CITATION = doi:10.1088/1475-7516/2007/12/011;%%
%131 citations counted in INSPIRE as of 10 Mar 2018
  
\bibitem{Biswas:2010zk} 
T.~Biswas, T.~Koivisto and A.~Mazumdar,
%``Towards a resolution of the cosmological singularity in non-local higher derivative theories of gravity,''
JCAP {\bf 1011}, 008 (2010)
doi:10.1088/1475-7516/2010/11/008
[arXiv:1005.0590 [hep-th]].
%%CITATION = doi:10.1088/1475-7516/2010/11/008;%%
%147 citations counted in INSPIRE as of 10 Mar 2018

\bibitem{Biswas:2012bp} 
T.~Biswas, A.~S.~Koshelev, A.~Mazumdar and S.~Y.~Vernov,
% ``Stable bounce and inflation in non-local higher derivative cosmology,''
JCAP {\bf 1208}, 024 (2012)
doi:10.1088/1475-7516/2012/08/024
[arXiv:1206.6374 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2012/08/024;%%
%111 citations counted in INSPIRE as of 10 Mar 2018
  
\bibitem{Koshelev:2012qn} 
A.~S.~Koshelev and S.~Y.~Vernov,
% ``On bouncing solutions in non-local gravity,''
Phys.\ Part.\ Nucl.\  {\bf 43}, 666 (2012)
doi:10.1134/S106377961205019X
[arXiv:1202.1289 [hep-th]].
%%CITATION = doi:10.1134/S106377961205019X;%%
%60 citations counted in INSPIRE as of 10 Mar 2018
  
\bibitem{Koshelev:2018rau} 
A.~S.~Koshelev, J.~Marto and A.~Mazumdar,
% "Towards resolution of anisotropic cosmological singularity in infinite derivative gravity,"
arXiv:1803.07072 [gr-qc].

%\cite{Buoninfante:2021xxl}
\bibitem{Buoninfante:2021xxl}
L.~Buoninfante,
%``Maximal Acceleration, Reciprocity \& Nonlocality,''
[arXiv:2105.08167 [hep-th]].
%0 citations counted in INSPIRE as of 15 Jun 2021


% %\cite{Koshelev:2016vhi}
% \bibitem{Koshelev:2016vhi}
% A.~S.~Koshelev, K.~Sravan Kumar and P.~Vargas Moniz,
% %``Effective models of inflation from a nonlocal framework,''
% Phys. Rev. D \textbf{96}, no.10, 103503 (2017)
% doi:10.1103/PhysRevD.96.103503
% [arXiv:1604.01440 [hep-th]].
% %22 citations counted in INSPIRE as of 20 Nov 2020

% %\cite{SravanKumar:2018dlo}
% \bibitem{SravanKumar:2018dlo}
% K.~Sravan Kumar and L.~Modesto,
% %``Non-local Starobinsky inflation in the light of future CMB,''
% [arXiv:1810.02345 [hep-th]].
% %8 citations counted in INSPIRE as of 20 Nov 2020

% %\cite{Koshelev:2020fok}
% \bibitem{Koshelev:2020fok}
% A.~S.~Koshelev and A.~Tokareva,
% %``Non-local self-healing of Higgs inflation,''
% [arXiv:2006.06641 [hep-th]].
% %1 citations counted in INSPIRE as of 20 Nov 2020

% %\cite{Koshelev:2020xby}
% \bibitem{Koshelev:2020xby}
% A.~S.~Koshelev, K.~S.~Kumar and A.~A.~Starobinsky,
% %``Analytic infinite derivative gravity, $R^2$-like inflation, quantum gravity and CMB,''
% Int. J. Mod. Phys. D \textbf{29}, 2043018 (2020)
% doi:10.1142/S021827182043018X
% [arXiv:2005.09550 [hep-th]].
% %5 citations counted in INSPIRE as of 20 Nov 2020

% %\cite{Koshelev:2020foq}
% \bibitem{Koshelev:2020foq}
% A.~S.~Koshelev, K.~Sravan Kumar, A.~Mazumdar and A.~A.~Starobinsky,
% %``Non-Gaussianities and tensor-to-scalar ratio in non-local R$^{2}$-like inflation,''
% JHEP \textbf{06}, 152 (2020)
% doi:10.1007/JHEP06(2020)152
% [arXiv:2003.00629 [hep-th]].
% %9 citations counted in INSPIRE as of 20 Nov 2020

  
%   %\cite{Ghoshal:2020lfd}
% \bibitem{Ghoshal:2020lfd}
% A.~Ghoshal, A.~Mazumdar, N.~Okada and D.~Villalba,
% %``Non-local Non-Abelian Gauge Theory: Conformal Invariance and $\beta$-function,''
% [arXiv:2010.15919 [hep-ph]].
% %0 citations counted in INSPIRE as of 11 Nov 2020

% %\cite{Ghoshal:2018gpq} 
% \bibitem{Ghoshal:2018gpq}
% A.~Ghoshal,
% %``Scalar dark matter probes the scale of nonlocality,''
% Int. J. Mod. Phys. A \textbf{34}, no.24, 1950130 (2019)
% doi:10.1142/S0217751X19501306
% [arXiv:1812.02314 [hep-ph]].
% %4 citations counted in INSPIRE as of 06 Mar 2021

% %\cite{Buoninfante:2018gce}
% \bibitem{Buoninfante:2018gce}
% L.~Buoninfante, A.~Ghoshal, G.~Lambiase and A.~Mazumdar,
% %``Transmutation of nonlocal scale in infinite derivative field theories,''
% Phys. Rev. D \textbf{99}, no.4, 044032 (2019)
% doi:10.1103/PhysRevD.99.044032
% [arXiv:1812.01441 [hep-th]].
% %20 citations counted in INSPIRE as of 06 Mar 2021

%\cite{Buoninfante:2018gce}
\bibitem{conference}
International Online Conference on Quantum Gravity, Higher-derivatives \& Nonlocalities, 8th to 12th March 2021,
\url{https://www.qgrav2021.com/}.




\bibitem{Coleman:1977py}
S.~R. Coleman, \emph{{Fate of the false vacuum: Semiclassical theory}},
  \href{https://doi.org/10.1103/PhysRevD.16.1248}{\emph{Phys. Rev. D}
  {\bfseries 15} (1977) 2929--2936}.
  
  %\cite{Callan:1977pt}
\bibitem{Callan:1977pt}
C.~G.~Callan, Jr. and S.~R.~Coleman,
%``The Fate of the False Vacuum. 2. First Quantum Corrections,''
Phys. Rev. D \textbf{16}, 1762-1768 (1977)
doi:10.1103/PhysRevD.16.1762
%1446 citations counted in INSPIRE as of 01 Mar 2022

%\cite{Kobzarev:1974cp}
\bibitem{Kobzarev:1974cp}
I.~Y.~Kobzarev, L.~B.~Okun and M.~B.~Voloshin,
%``Bubbles in Metastable Vacuum,''
Yad. Fiz. \textbf{20}, 1229-1234 (1974)
ITEP-81-1974.
%419 citations counted in INSPIRE as of 02 Mar 2022

%\cite{Croon:2021vtc}
\bibitem{Croon:2021vtc}
D.~Croon, E.~Hall and H.~Murayama,
%``Non-perturbative methods for false vacuum decay,''
[arXiv:2104.10687 [hep-th]].
%4 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Frasca:2022kfy}Croon:2021vtc
\bibitem{Frasca:2022kfy}
M.~Frasca, A.~Ghoshal and N.~Okada,
%``Fate of False Vacuum in Non-perturbative Regimes,''
[arXiv:2201.12267 [hep-th]].
%2 citations counted in INSPIRE as of 03 Mar 2022

\bibitem{Coleman:1980aw}
S.~R. Coleman and F.~De~Luccia, \emph{{Gravitational effects on and of vacuum
  decay}}, \href{https://doi.org/10.1103/PhysRevD.21.3305}{\emph{Phys. Rev. D}
  {\bfseries 21} (1980) 3305}.
 
  
  
  %\cite{Coleman:1987rm}
\bibitem{Coleman:1987rm}
S.~R.~Coleman,
%``Quantum Tunneling and Negative Eigenvalues,''
Nucl. Phys. B \textbf{298}, 178-186 (1988)
doi:10.1016/0550-3213(88)90308-2
%150 citations counted in INSPIRE as of 01 Mar 2022

\bibitem{Calcagni:2007ef}
G.~Calcagni, M.~Montobbio and G.~Nardelli, \emph{{Localization of nonlocal
  theories}}, \href{https://doi.org/10.1016/j.physletb.2008.03.024}{\emph{Phys.
  Lett. B} {\bfseries 662} (2008) 285--289},
  [\href{https://arxiv.org/abs/0712.2237}{{\ttfamily 0712.2237}}].

\bibitem{Calcagni:2008nm}
G.~Calcagni and G.~Nardelli, \emph{{Nonlocal instantons and solitons in string
  models}}, \href{https://doi.org/10.1016/j.physletb.2008.09.016}{\emph{Phys.
  Lett. B} {\bfseries 669} (2008) 102--106},
  [\href{https://arxiv.org/abs/0802.4395}{{\ttfamily 0802.4395}}].

\bibitem{Calcagni:2009jb}
G.~Calcagni and G.~Nardelli, \emph{{String theory as a diffusing system}},
  \href{https://doi.org/10.1007/JHEP02(2010)093}{\emph{JHEP} {\bfseries 02}
  (2010) 093}, [\href{https://arxiv.org/abs/0910.2160}{{\ttfamily 0910.2160}}].

\bibitem{Calcagni:2018lyd}
G.~Calcagni, L.~Modesto and G.~Nardelli, \emph{{Initial conditions and degrees
  of freedom of non-local gravity}},
  \href{https://doi.org/10.1007/JHEP05(2018)087}{\emph{JHEP} {\bfseries 05}
  (2018) 087}, [\href{https://arxiv.org/abs/1803.00561}{{\ttfamily
  1803.00561}}].

\bibitem{Calcagni:2018fid}
G.~Calcagni, \emph{{Taming the Beast: Diffusion Method in Nonlocal Gravity}},
  \href{https://doi.org/10.3390/universe4090095}{\emph{Universe} {\bfseries 4}
  (2018) 95}, [\href{https://arxiv.org/abs/1809.04292}{{\ttfamily
  1809.04292}}].
  
  %\cite{Barman:2021lot}
\bibitem{Barman:2021lot}
B.~Barman and A.~Ghoshal,
%``Scale Invariant FIMP Miracle,''
[arXiv:2109.03259 [hep-ph]].
%3 citations counted in INSPIRE as of 03 Mar 2022
  
  
  %\cite{Ghoshal:2022hyc}
\bibitem{Ghoshal:2022hyc}
A.~Ghoshal, N.~Okada and A.~Paul,
%``Radiative Plateau Inflation with Conformal Invariance: Dynamical Generation of Electroweak and Seesaw Scales,''
[arXiv:2203.00677 [hep-ph]].
%0 citations counted in INSPIRE as of 03 Mar 2022
  
  %\cite{Edholm:2016hbt}
\bibitem{Edholm:2016hbt}
J.~Edholm, A.~S.~Koshelev and A.~Mazumdar,
%``Behavior of the Newtonian potential for ghost-free gravity and singularity-free gravity,''
Phys. Rev. D \textbf{94}, no.10, 104033 (2016)
doi:10.1103/PhysRevD.94.104033
[arXiv:1604.01989 [gr-qc]].
%108 citations counted in INSPIRE as of 02 Mar 2022

%\cite{LIGOScientific:2019vic}
\bibitem{LIGOScientific:2019vic}
B.~P.~Abbott \textit{et al.} [LIGO Scientific and Virgo],
%``Search for the isotropic stochastic background using data from Advanced LIGO\textquoteright{}s second observing run,''
Phys. Rev. D \textbf{100}, no.6, 061101 (2019)
doi:10.1103/PhysRevD.100.061101
[arXiv:1903.02886 [gr-qc]].
%197 citations counted in INSPIRE as of 03 Mar 2022


%\cite{Romero:2021kby}
\bibitem{Romero:2021kby}
A.~Romero, K.~Martinovic, T.~A.~Callister, H.~K.~Guo, M.~Mart\'\i{}nez, M.~Sakellariadou, F.~W.~Yang and Y.~Zhao,
%``Implications for First-Order Cosmological Phase Transitions from the Third LIGO-Virgo Observing Run,''
Phys. Rev. Lett. \textbf{126}, no.15, 151301 (2021)
doi:10.1103/PhysRevLett.126.151301
[arXiv:2102.01714 [hep-ph]].
%17 citations counted in INSPIRE as of 03 Mar 2022

%\cite{KAGRA:2021mth}
\bibitem{KAGRA:2021mth}
R.~Abbott \textit{et al.} [KAGRA, Virgo and LIGO Scientific],
%``Search for anisotropic gravitational-wave backgrounds using data from Advanced LIGO and Advanced Virgo\textquoteright{}s first three observing runs,''
Phys. Rev. D \textbf{104}, no.2, 022005 (2021)
doi:10.1103/PhysRevD.104.022005
[arXiv:2103.08520 [gr-qc]].
%28 citations counted in INSPIRE as of 03 Mar 2022

%\cite{Nortier:2021six}
\bibitem{Nortier:2021six}
F.~Nortier,
%``Shadow Extra Dimensions \& Fuzzy Branes with an Exorcized Spectrum,''
[arXiv:2112.15592 [hep-th]].

%\cite{Grinstein:2007mp}
\bibitem{Grinstein:2007mp}
B.~Grinstein, D.~O'Connell and M.~B.~Wise,
%``The Lee-Wick standard model,''
Phys. Rev. D \textbf{77} (2008), 025012
doi:10.1103/PhysRevD.77.025012
[arXiv:0704.1845 [hep-ph]].

%\cite{Carone:2008iw}
\bibitem{Carone:2008iw}
C.~D.~Carone and R.~F.~Lebed,
%``A Higher-Derivative Lee-Wick Standard Model,''
JHEP \textbf{01} (2009), 043
doi:10.1088/1126-6708/2009/01/043
[arXiv:0811.4150 [hep-ph]].

%\cite{Buoninfante:2017kgj}
\bibitem{Buoninfante:2017kgj}
L.~Buoninfante, G.~Lambiase and A.~Mazumdar,
%``Quantum solitonic wave-packet of a meso-scopic system in singularity free gravity,''
Nucl. Phys. B \textbf{931}, 250-261 (2018)
doi:10.1016/j.nuclphysb.2018.04.012
[arXiv:1708.06731 [quant-ph]].

\cite{Buoninfante:2017rbw}
\bibitem{Buoninfante:2017rbw}
L.~Buoninfante, G.~Lambiase and A.~Mazumdar,
%``Quantum spreading of a self-gravitating wave-packet in singularity free gravity,''
Eur. Phys. J. C \textbf{78}, no.1, 73 (2018)
doi:10.1140/epjc/s10052-018-5535-4
[arXiv:1709.09263 [gr-qc]].

%\cite{Buoninfante:2019teo}
\bibitem{Buoninfante:2019teo}
L.~Buoninfante, A.~Mazumdar and J.~Peng,
%``Nonlocality amplifies echoes,''
Phys. Rev. D \textbf{100}, no.10, 104059 (2019)
doi:10.1103/PhysRevD.100.104059
[arXiv:1906.03624 [gr-qc]].


%\end{thebibliography}
\end{thebibliography}
\endgroup
